RMM: A Recursive Mental Model for Dialog Navigation

Language-guided robots must be able to both ask humans questions and understand answers. Much existing work focuses only on the latter. In this paper, we go beyond instruction following and introduce a two-agent task where one agent navigates and asks questions that a second, guiding agent answers. Inspired by theory of mind, we propose the Recursive Mental Model (RMM). The navigating agent models the guiding agent to simulate answers given candidate generated questions. The guiding agent in turn models the navigating agent to simulate navigation steps it would take to generate answers. We use the progress agents make towards the goal as a reinforcement learning reward signal to directly inform not only navigation actions, but also both question and answer generation. We demonstrate that RMM enables better generalization to novel environments. Interlocutor modelling may be a way forward for human-agent dialogue where robots need to both ask and answer questions.

==> Dialogue Navigation/01-introduction.tex <==

\section{Introduction}
A key challenge for embodied language is moving beyond instruction following to instruction generation, which can require understanding the listener.
The turn-based \dia{} paradigm raises a myriad of new research questions, from grounded versions of traditional problems like co-reference resolution \cite{visual_dialogue} to explicitly modeling theory of mind in order to consider the listener's ability to understand generated instructions~\cite{Bisk2020}.
In this paper, we develop end-to-end \dia{} agents to navigate photorealistic, indoor scenes to reach goal rooms.
We train agents using the human-human Collaborative Vision-and-\Dia{} Navigation (CVDN)~\cite{cvdn} dataset.
CVDN \dias{} are turn-based, with a \textit{navigator} following \textit{guide} instructions and asking questions when needed.

\newpage
Modeling turn-based \dias{} involves four core challenges:
\begin{enumerate}[noitemsep,nolistsep,label={\bfseries C\arabic*}]
\item \label{ch:ask} A \textit{navigator} deciding when to ask a question.
\item \label{ch:que} Generating \textit{navigator} questions.
\item \label{ch:ans} Generating \textit{guide} question answers.
\item \label{ch:act} Generating \textit{navigator} actions.
\end{enumerate}

Prior work has addressed individual components of turn-based \dia\ modeling.
This work is the first to train \textit{navigator} and \textit{guide} agents to perform end-to-end, collaborative \dia{}s with question generation (\ref{ch:que}), question answering (\ref{ch:ans}), and navigation (\ref{ch:act}) conditioned on \dia{} history.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/Fig1-Robot.pdf}
    \caption{The \acronym{} agent recursively models conversations with instances of itself to choose the right questions to ask (and answers to give) to reach the goal.}
    \label{fig:rmm}
\end{figure}

Theory of mind~\cite{theory_of_mind_child} posits that efficient questions and answers build on a shared world of experiences and referents.
To communicate efficiently, people model both a listener's mental state and the effects of their actions on the world.
Modeling future worlds in navigation~\cite{ghosts} and control~\cite{prospection} are open research questions, and we approximate solutions through a \approach{} (\acronym) of a conversational partner.
Our agent spawns instances of \textit{itself} to simulate the effects of \dia{} acts \textit{before} asking a question or generating an answer to estimate their effects on navigation.
Viewed as a single system, the agents cooperatively search through the space of \dia{}s to efficiently perform embodied navigation.

==> Dialogue Navigation/02-related.tex <==
\section{Related Work and Background}
We build on research in multimodal navigation and the wider literature involving goal oriented \dia.
Table~\ref{tab:dialogue_challenges} summarizes how our work differs from existing work in vision-and-language navigation and task-oriented dialogue modelling.



\paragraph{Instruction Following} tasks an embodied agent with interpreting natural language instructions and visual observations to reach a goal~\cite{jayannavar-etal-2020-learning,self_supervised_imitation_learning,ma2019b,vln,interpret_instructions}.
These instructions describe step-by-step actions the agent needs to take, and can involve the creation of speaker models for data augmentation that provide additional instructions~\cite{speaker-follower}.
This paradigm has been extended to longer trajectories and outdoor environments \cite{vln_streets}, as well as to agents in the real world~\cite{language_to_action, inverse_semantics}.
In this work, we focus on the the simulated, photorealistic indoor environments of the MatterPort dataset \cite{matterport}, and go beyond instruction following alone to a two-agent \dia{} setting.

\paragraph{Navigation \Dia{}s} task a \textit{navigator} and a \textit{guide} to cooperate to find a destination.
Previous work includes substantial information asymmetry between the navigator and guide~\cite{talk_the_walk,narayan-chen-etal-2019-collaborative}.
Information asymmetry can take the form of the \textit{navigator} seeing a bird's eye, abstract semantic map while the \textit{guide} sees egocentric simulation frames~\cite{talk_the_walk}, affecting the kind of dialog possible when low-level visual cues cannot be grounded by the \textit{navigator}.
Other work only investigates the \textit{navigation} portion of the \dia{} without considering text question generation and answering~\cite{cvdn}.
Going beyond models that perform navigation from \dia{} history alone~\cite{Wang:2020,Zhu:2020,Hao:2020}, or decide when to ask \emph{navigator} questions but do so as a simple ``help'' flag with oracle responses~\cite{chi:aaai20,nguyen2019vnla}, in this work we train two agents: a navigator agent that asks questions, and a guide agent that answers those questions.

\begin{table}
\begin{tabular}{@{}p{0.29\textwidth}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{}}
    \bf Representative Work & \ref{ch:ask} & \ref{ch:que} & \ref{ch:ans} & \ref{ch:act} \\
    \toprule
    \citet{vln} & \xmark & \xmark & \xmark & \cmark \\
    \citet{speaker-follower} & \xmark & \xmark & \cmark & \cmark \\
    \citet{narayan-chen-etal-2019-collaborative} & \xmark & \xmark & \cmark & \xmark \\
    \citet{nguyen2019hanna} & \cmark & \xmark & \cmark & \cmark \\
    \citet{chi:aaai20} & \cmark & \xmark & \xmark & \cmark \\
    \citet{cvdn} & \xmark & \xmark & \xmark & \cmark \\
    \midrule
    RMM & \xmark & \cmark & \cmark & \cmark \\
    \bottomrule
\end{tabular}
\caption{Previous work has addressed subsets of the four key challenges for turn-based navigation \dias{} by training single-turn agents.
No prior work has tackled generating \emph{navigator} questions (\ref{ch:que}); by doing so, our work becomes the first to train two agents jointly on multi-turn \dias{} where agents both produce and consume task-relevant language.
We eschew only the challenge of deciding \textit{when} to ask questions (\ref{ch:ask}), using a fixed heuristic instead.}
\label{tab:dialogue_challenges}
\end{table}


\paragraph{Multimodal \Dia{}} takes several forms.
In Visual \Dia{}~\cite{visual_dialogue}, an agent answers a series of questions about an image that may require \dia{} context.
Reinforcement learning gives strong performance on this task~\cite{visdial_rl}, and such paradigms have been extended to producing multi-domain visual \dia{} agents~\cite{Ju2019AllinOneIC}.
GuessWhat~\cite{Vries2017a} presents a similar paradigm, where agents use visual properties of objects to reason about which referent meets various constraints.
Identifying visual attributes can also lead to emergent communication between pairs of learning agents~\cite{cao2018emergent}.

\paragraph{Goal Oriented \Dia} systems can help a user achieve a predefined goal, from booking flights to learning kitchen tasks \citep{taskorientedgao,2015serbansurvey,bordesweston2017,language_to_action}.
Modeling goal-oriented \dia{} requires skills that go beyond language modeling, such as asking questions to clearly define a user request, querying knowledge bases, and interpreting results from queries as options to complete a transaction.
Many recent task oriented systems are data-driven and trained end-to-end using semi-supervised or transfer learning methods \citep{gpt2dialog,neuralbelieftracker}. 
However, these data-driven approaches may lack grounding between the text and the environment state.
Reinforcement learning-based \dia{} modeling~\cite{rewardshaping,deeprlfordialog,deeprlfordialog1} can improve completion rate and user experience by helping ground conversational data to environments.


==> Dialogue Navigation/03-task.tex <==
\section{Task and Data}

Our work creates a two-agent \dia{} task, building on the CVDN dataset~\cite{cvdn} of human-human \dia s.
In that dataset, a human \Nr{} and \Or{} collaborate to find a goal room containing a target object.
The \Nr{} moves through the environment, and the \Or{} views this navigation until the \Nr{} asks a question in natural language (\ref{ch:ask}, \ref{ch:que}).
Then, the \Or{} can see the next few steps a shortest path planner would take towards the goal, and produces a natural language response (\ref{ch:ans}).
\Dia{} continues until the \Nr{} arrives at the goal (\ref{ch:act}).

\noindent We model this \dia{} between two agents:
\begin{enumerate}[noitemsep,nolistsep]
    \item Questioner ($\mathcal{Q}$) \& Navigator ($\mathcal{N}$)
    \item Guide ($\mathcal{G}$)
\end{enumerate}
We split the first agent into its two roles: question asking (\ref{ch:que}) and navigation (\ref{ch:act}).
As input, the agents receive the same data as their human counterparts in CVDN.
Specifically, both agents (and all three roles) have access to the entire \dia{} and visual navigation histories, in addition to a textual description of the target object (e.g., \textit{a plant}). 
The \Nr{} uses this information to execute on a sequence of actions composed of: \texttt{forward}, \texttt{left}, \texttt{right}, \texttt{look up}, \texttt{look down}, and \texttt{stop}.
The \Qr{} asks for specific guidance from the \Or.
The \Or{} is presented with the navigation and \dia{} histories as well as the next five shortest path steps to the goal, given as a sequence of image observations those steps produce.

Agents are trained on human-human \dia{}s of natural language questions and answers from CVDN.
Individual question-answer exchanges in that dataset are underspecified and rarely provide simple step-by-step instructions like ``straight, straight, right, ...''.
Instead, exchanges rely on assumptions of world knowledge and shared context~\cite{pragmatic_reasoning, logic_and_conversation}, which manifest as instructions rich with visual-linguistic co-references such as \textit{should I go back to the room I just passed or continue on?} 

\begin{algorithm}[t]
\begin{small}
\SetAlgoLined
 $loc = p_0$\;
 $hist = t_0$\;
 $\vec{a} \sim \mathcal{N}(hist)$\;
 $loc, hist = \mathrm{update(}\vec{a}, loc, hist)$\;
 \While{$\vec{a} \neq$ \texttt{STOP} \textbf{and} $len(hist) < 20$}{
  $q \sim \mathcal{Q}(hist, loc)$ \tcp*{Question}
  $\vec{s} = \mathrm{path(}loc, goal\mathrm{, horizon=5)}$ \;
  $o \sim \mathcal{O}(hist, loc, q, \vec{s})$ \tcp*{Answer}
  $hist \leftarrow hist + (q,o)$\;
  \For{$a \in \mathcal{N}(hist)$}{
     $loc \leftarrow loc + a$      \tcp*{Move}
     $hist \leftarrow hist + a$\;
  }
 }
 return $(goal - t_0) - (loc - t_0)$
 \end{small}
 \caption{\Dia{} Navigation}
 \label{alg:dialogue-navigation}
\end{algorithm}


The CVDN release does not provide any baselines or evaluations for the interactive \dia{} setting we present, and instead focuses solely on navigation (\ref{ch:act}).
We use the same metric as that work, ``Goal Progress" in meters---the distance reduction between the \Nr{}'s starting position and ending position with respect to the goal location.

\Dia{} navigation proceeds by iterating through the three roles until either the \Nr{} chooses to stop or a maximum number of turns are played (Algorithm \ref{alg:dialogue-navigation}).
In addition to ``Goal Progress'', we report BLEU scores \cite{papineni-etal-2002-bleu} for evaluating the generation of questions and answers by comparing against human questions and answers. Note, in our \dia{} setting, Goal Progress also implicitly measures the utility of generated language and is therefore complementary to BLEU when evaluating utility versus fluency.


==> Dialogue Navigation/04-model.tex <==

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/ActionDecoder.pdf}
        \caption{\Dia{} and action histories combined with the current observation are used to predict the next navigation action.}
        \label{fig:action_decoder}
    \end{subfigure}%
    \hspace{1em} 
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{images/LanguageDecoder.pdf}
        \caption{\Or{} Bi-LSTM over the path is attended to during decoding for answer generation.}
        \label{fig:language_decoder}
    \end{subfigure}
        \caption{Our backbone Seq2Seq architectures are provided visual observations and portions of the \dia{} history when taking actions or asking/answering questions.}
        \label{fig:models}
\end{figure*}

\section{Models}
We introduce the \approach{} (\acronym) as an initial approach to our new full \dia{} CVDN task formulation.
Key to this approach is allowing component models (\Nr{}, \Qr{}, and \Or{}) to learn from each other and roll out possible \dia{}s and trajectories.
We compare our model to a traditional sequence-to-sequence baseline, and we explore data augmentation using the Speaker-Follower method~\cite{speaker-follower}.

\subsection{Sequence-to-Sequence Architecture}
The underlying architecture, shown in Figure \ref{fig:models}, is shared across all approaches.
The core \dia{} tasks are navigation action decoding and language generation for asking and answering questions.
We present three sequence-to-sequence \cite{attention_mechanism} models to perform as \Nr, \Qr, and \Or.
The models rely on an LSTM \cite{lstm} encoder for the \dia{} history.
To encode visual observations, our models take the penultimate ResNet~\cite{resnet} layer as the image observation.
Future work may explore different and more nuanced encoding architectures.

\paragraph{Navigation Action Decoding (\ref{ch:act})}
Initially, the \dia{} context is just a target object \target{} category, for example ``plant.''
The goal room contains an instance of that category.
As questions are asked and answered, the \dia{} context grows.
Following prior work~\cite{vln,cvdn}, \dia{} history words $\vec{w}$ words are embedded as 256 dimensional vectors and passed through an LSTM to produce $\vec{u}$ context vectors and a final hidden state $h_N$.
The hidden state $h_N$ is used to initialize the LSTM decoder.
At every timestep the decoder is updated with the previous action $a_{t-1}$ and current image observation $I_{t}$.
The hidden state is used to attend over the language $\vec{u}$ and predict the next action $a_t$ (Figure \ref{fig:action_decoder}).

We pretrain the \Nr{} on the navigation task alone before fine-tuning in the full \dia{} setting that we introduce.
The next action is sampled from the model's predicted logits, and the episode ends when either a \texttt{stop} action is sampled or 80 actions are taken~\cite{cvdn}.  

\paragraph{Speaker Models (\ref{ch:que} \& \ref{ch:ans})}
To generate questions and answers, we train sequence-to-sequence models (Figure \ref{fig:language_decoder}) where an encoder takes in a sequence of images and a decoder produces a sequence of word tokens.
At each decoding timestep, the decoder attends over the input images to predict the next word of the question or answer.
This model is also initialized via training on CVDN \dia{}s.
In particular, question asking (\Qr) encodes the images of the current viewpoint where a question is asked, and then decodes the question tokens produced by the human \Nr.
Question answering (\Or) encodes images of the next five steps the shortest path planner would take towards the goal, then decodes the language tokens produced by the human \Or.
Pretraining initializes the lexical embeddings and attention alignments before fine-tuning in the collaborative, turn-taking setting we introduce in this paper.

\paragraph{Conditioning Context}
We define three levels of \dia{} context given as input to our \Nr{} agents in order to evaluate how well they utilize the generated conversations.
We compare agents' ability to navigate to the goal room given:

\begin{itemize}[align=parleft, labelsep=2em,leftmargin =\dimexpr\labelwidth+\labelsep\relax]
    \item[\target] the target object present in the goal room;
    \item[\QA] additionally the previous question-and-answer exchange;
    \item[\QAfull] additionally the entire \dia{} history.
\end{itemize}

We constrain the \Qr{} and \Or{} speaker models to condition on fixed contexts.
The \Qr{} model 
takes as input the current visual observation $I_t$ and the target object $t_O$.
The \Or{} model 
takes 
the visual observations $I^*_{t+1:t+5}$ of the next five steps of navigation according to a shortest path planner, the target object $t_O$, and the last question $Q_{i-1}$ generated by the \Qr{}.\footnote{This limits phenomena like co-reference, but dramatically reduces the model's input space.  Handling arbitrarily long contexts with limited training data is left to future work.}

\subsection{\approach}
We introduce the \approach{} agent (\acronym),\footnote{\url{https://github.com/HomeroRR/rmm}}
which is trained with reinforcement learning to propagate feedback from navigation error through all three component models: \Nr{}, \Qr{}, and \Or{}.
In this way, the training signal for question generation includes the training signal for answer generation, which in turn is derived from the training signal from navigation error.
The agent's progress towards the goal in the environment informs the \dia{} itself; each model educates the others (Figure \ref{fig:rl_recursive}).

Each model among the \Nr{}, \Qr{}, and \Or{} may sample $N$ trajectories or generations of max length $L$.
These samples in turn are considered recursively by the \acronym{} agent, leading to $N^T$ possible \dia{} trajectories, where $T$ is at most the maximum trajectory length.
To prevent unbounded exponential growth during training, each model is limited to a maximum number of total recursive calls per run.
Search techniques, such as frontiers \cite{Ke2019}, could be employed in future work to guide the agent.

\paragraph{Training}
In the \dia{} task we introduce, the agents begin only knowing the name of the target object.
The \Nr{} agent must move towards the goal room containing the target object, and can ask questions using the \Qr{} model.
The \Or{} agent answers those questions given a privileged view of the next steps in the shortest path to the goal rendered as visual observations.

We define two different loss functions to learn the parameters $\theta$ of the \Nr{}  agent.
We learn a policy $\pi_\theta(\tau|t_O)$ which maximizes the log-likelihood of the shortest path trajectory $\tau$ given target object $t_O$ present in the goal room (Eq. \ref{eq:goal}).
The action decoder $\textbf{a}_t = \textit{f}_{\theta_D}(\textbf{z}_t,I_t)$ takes language encoder $\textbf{z}_t  = \textit{f}_{\theta_E}(w_{1:t})$ as input along with the image observations $I_t$ at time $t$.
\Dia{} context at time $t$, $w_{1:t}$ is input to the language encoder. The cross entropy loss is defined as:
\begin{align}
  J_{CE}(\theta) & = -\sum_{t=1}^{T} log \ \pi_\theta(\textbf{a}_t|I_t, t_O, w_{1:t}) \label{eq:goal}
\end{align}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/qgn_recursive.pdf}
\caption{The \approach{} allows for each sampled generation to spawn a new \dia{} and corresponding trajectory to the goal.  The \dia{} that leads to the most goal progress is followed by the agent.}
\label{fig:rl_recursive}
\end{figure}

Our second \Nr{} RL agent loss is standard policy gradient based Advantage Actor Critic~\cite{rl} 
minimizing a k-step TD\footnote{Temporal Difference} error of the critic, $J_{RL}(\theta)$:
\begin{align}
  = & -\ \sum_{t=1}^{T} \textbf{A}^\pi \ log \ \pi_\theta(\textbf{a}_t|I_t, t_O, w_{1:t}) + \frac{1}{2}\sum_{t=1}^{T} (\textbf{A}^\pi)^2 \label{eq:a2c}
\end{align}
 
\noindent $\textbf{A}^\pi$=$r_{t+1}$+$V^\pi(I_{t+1})$-$V^\pi(I_t)$ is the advantage function in Eq. \ref{eq:a2c}, where
$r_{t+1}$ is the reward measured by the goal progress and the $V^\pi$ denotes the state-value (critic) model. The first term in Eq. \ref{eq:a2c} is the actor loss, while the second term is the critic (value) loss of the advantage actor critic loss function. 
The overall system is trained end-to-end using sum of the RL agent loss of the navigator agent $J_{RL}(\theta)$ and the  cross entropy loss between the ground truth and the generated trajectories, $J_{CE}(\theta)$. 
The speaker model parameters are also updated via the sum of the standard question/answer generation cross entropy and the composite \Nr{} agent loss from the branch with the max goal progress. 
 
\paragraph{Inference}
\label{sec:inference}
During training, exact environmental feedback---the remaining distance to the goal---can be used to evaluate samples and trajectories.
This information is not available during inference, so we instead rely on the navigator's confidence to determine which of several sampled paths should be explored.
For every question-answer pair sampled, the agent rolls forward five navigation actions per sequence, and the trajectory sequence with the highest probability is used for the next timestep.
This heuristic does not guarantee that the model is progressing towards the goal, but empirically confidence-based estimation enables progress.


\subsection{\Dia{} Gameplay}
As is common in \dia{} settings, there are several moving pieces and a growing notion of state throughout training and evaluation.
In addition to the \Nr{}, \Qr{}, and \Or{}, the \Nr{} agent also needs to determine when to invoke the \Qr{} model to get supervision from the \Or{} (\ref{ch:ask}).
We leave this component---when to ask questions---for future work and set a fixed number of steps before asking a question.
We invoke the \Qr{} model after every $4$ navigation steps based on the human average of $4.5$ steps between questions in CVDN.

Setting a maximum trajectory length is required due to computational constraints as the the language context $w_{1:j}$ grows.
Following \citet{cvdn}, we use a maximum navigation length of 80 steps, leading to a maximum of $\frac{80}{4} = 20$ question-answer exchanges per \dia{}.

We use a single model for question and answer generation, and indicate the role of spans of text by prepending \texttt{<NAV>} (\Qr{} navigation questions) or \texttt{<ORA>} (\Or{} answers based on oracle views) tags (Figure~\ref{fig:action_decoder}) to condition the generation task.
During roll outs the model is reinitialized to prevent information sharing via the hidden units.

\subsection{Training Details}
\label{ssec:training}

We initialize the \Nr{}, \Qr{}, and \Or{} agents as encoder-decoder LSTM models with 512 hidden dimensions.
The \Nr{} encoder is a forward LSTM, while the \Qr{} and \Or{} speaker models use bi-LSTM encoders.
We use the 512 dimensional penultimate ResNet layer for image observations $I_t$, embed words $w$ in 256 dimensions, and embed actions in $32$ dimensions.
The models observe a word history up to $160$ tokens, and can decode up to $80$ actions per episode.
The value/critic module is a linear layer with relu and dropout on top of the hidden state. 

We optimize the \Nr{} models with the Adam optimizer~\cite{kingma:iclr15} with a learning rate of $0.0001$ with weight decay $0.0005$.
For the \Qr{} and \Or{} models, we use an RMSProp optimizer with learning rate $0.0001$.

Models are pretrained on CVDN data with batches of size $100$ for $20,000$ iterations.
During self-play, models are trained with batches of $10$, for \acronym{} with $N=3$, or $100$ else for $5,000$ iterations.
A dropout rate of $0.5$ is used during all training.
All \Nr{} models are trained using student sampling~\cite{vln}. 
In \acronym$_{N=3}$, one action sequence is produced via argmax decoding, while the other two via sampling (no temperature).  The same is true for language decoding but with a temperature of 0.6.  Exploration of how sampler strategies effect performance is left for future work.

\paragraph{Data Augmentation (DA)}
Navigation agents can benefit from generated language instructions~\cite{speaker-follower}.
We augment the baseline model's navigation training data in a fashion similar to the rollouts of \acronym$_{N=3}$ to create a more direct comparison between the baseline and \acronym.
We choose a CVDN conversation 
and sample three action trajectory rollouts, two by sampling an action at each timestep, and one by taking the argmax action at each timestep.
We evaluate those trajectories' progress towards the conversation goal location and keep the best for augmentation.
We give the visual observations of the chosen path to the pretrained \Qr{} model to produce a relevant instruction.
This trajectory paired with a generated language instruction is added to the training data, and we 
downweight the contributions of these noisier pairs to the overall loss, so $loss = \lambda * \text{generations} + (1-\lambda) * \text{human}$.
The choice of $\lambda$ affects the fluency of the language generated;
we use $\lambda=0.1$.


==> Dialogue Navigation/05-results.tex <==
\begin{table}
\centering
\begin{small}
\begin{tabular}{@{}l@{\hspace{2pt}}l@{\hspace{5pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}a@{\hspace{2pt}}c@{\hspace{7pt}}c@{\hspace{2pt}}a@{}}
 & \textbf{Model} &               \multicolumn{4}{@{}c@{}}{\textbf{Goal Progress (m) $\uparrow$}} & \multicolumn{2}{c}{\textbf{\textbf{BLEU} $\uparrow$}} \\
\toprule
  &  & \begin{scriptsize}\target\end{scriptsize}& \begin{scriptsize}\QA\end{scriptsize}& \begin{scriptsize}\QAfull\end{scriptsize}& \begin{scriptsize}\begin{tabular}{@{}c@{}}+\! Oracle\\Stopping\end{tabular}\end{scriptsize} & \begin{scriptsize}\QA\end{scriptsize}& \begin{scriptsize}\QAfull\end{scriptsize}\\
  \midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{Val Seen}}  
& Seq2Seq          & \textbf{20.1}& 10.5      & \Be{15.0}     & \textbf{22.9} & 0.9    & 0.8     \\
& Seq2Seq  + DA    &  20.1    & 10.5      & 10.0     & 14.2 & 1.3    & 1.3     \\
& \acronym$_{N=1}$ & 18.7     & 10.0      & 13.3     & 20.4 & 3.3    & 3.0     \\
& \acronym$_{N=3}$ & 18.9     & \textbf{11.5} & 14.0 & 16.8 &\textbf{3.4}&\Be{3.6}\\
&  Shortest Path   &  \multicolumn{4}{@{}c@{}}{----------- 32.8 ----------- }    &   & \cellcolor{white}\\
\midrule
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{Val Unseen}}    
& Seq2Seq          & 6.8     & 4.7      & \PZ4.6      & 6.3& 0.5  & 0.5\\
& Seq2Seq + DA     & 6.8     & 5.6      & \PZ4.4      & 6.5& 1.3  & 1.1\\
& \acronym$_{N=1}$ & 6.1     &\textbf{6.1}  & \PZ5.1      & 6.0 & 2.6  & 2.8\\
& \acronym$_{N=3}$ &\textbf{7.3} & 5.5      & \PZ\Be{5.6} &\textbf{8.9} &\textbf{2.9}&\Be{2.9}\\
& Shortest Path    & \multicolumn{4}{@{}c@{}}{----------- 29.3 ------------}                & & \cellcolor{white} \\
\bottomrule
\end{tabular}
\end{small}
\caption{\Dia{} results on CVDN.
Data Augmentation adds noisy training data for the model.
Goal progress evaluates the quality of the inferred navigation trajectory, while BLEU scores estimate the quality of the generated questions and answers.
Evaluations conditioning on the entire \dia{} history are highlighted in \colorbox{gray!20}{gray} with the best results in \Be{blue}.
}
\label{table:cvdn_results}
\end{table}



\section{Results}
\label{section:results}
In Table \ref{table:cvdn_results} we present \dia{} results for our \acronym{} agent and competitive baselines.
We report two main results and four ablations for \textit{seen} and \textit{unseen} house evaluations; the former are novel \dia{}s in houses seen at training time, while the latter are novel \dia{}s in novel houses.

\paragraph{Full Evaluation}
The full evaluation paradigm conditions navigation on the entire \dia{} history \QAfull{} in addition to the original target object \target.
We present two conditions for \acronym{} ($N=1$ and $N=3$).
Recall that $N$ indicates the number of trajectories (\Nr{}) or generations (\Qr{}, \Or{}) explored in our recursive calls.
$N=1$ corresponds to taking the single maximum prediction while $N=3$ allows the agent to sample alternatives (Section \ref{sec:inference}).
While low, the BLEU scores are better for \acronym{}-based agents across settings.

A challenge for navigation agents is knowing when to \texttt{stop}.
Following previous work~\cite{vln}, we additionally report Oracle Success Rates measuring the best goal progress the agents achieve along the trajectory.

In \textit{unseen} environments, the \acronym{}-based agents make the most progress towards the goal and benefit from exploration at during inference ($N=3$), and this result holds when considering Oracle Success.
In \textit{seen} environments, by contrast, the \acronym{}-based agents perform slightly less well than the baseline sequence-to-sequence models on goal progress.
This effect may be a consequence of \textit{environment bias} in navigation simulations where houses are seen at both training and inference time with overlapping paths~\cite{zhang:ijcai20}.


\paragraph{Ablations}
We also include two simpler results: \target, where the agent is only provided the target object and explores based on this simple goal, and \QA{} where the agent is only provided the previous question-answer pair.
Both of these settings simplify the learning and evaluation by focusing the agent on search and less ambiguous language, respectively.
There are two results to note.

First, given only \target{} the \acronym{} trained model with sampling generalizes best to \textit{unseen} environments.
In this setting, during inference all models have the same limited information, so the RL loss and exploration have better equipped \acronym{} to generalize.

Second, several trends invert between the \textit{seen} and \textit{unseen} scenarios.
Specifically, the simplest model with the least information performs best overall in \textit{seen} houses.
This high performance coupled with weak language appears to indicate the models are learning a different (perhaps search based) strategy rather than how to utilize \dia{}.
In the \QA{} and \QAfull{} settings, the agent generates a question-answer pair before navigating, so the relative strength of the \acronym{} model's communication becomes clear.
We analyze the generated language and navigation behavior of our models.


\begin{figure}[t]
\includegraphics[width=\columnwidth]{images/lex_dist.pdf}
\caption{Log-frequency of words generated by human speakers as compared to the Data Augmentation (DA) 
and our \approach{} (\acronymnormal{}) models.}
\label{fig:lexdist}
\end{figure}


==> Dialogue Navigation/06-analysis.tex <==

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/GoalQs.pdf}
        \caption{Human goal progress as \dia{}s unfold.
        As humans ask questions and make goal guesses, they roughly linearly make progress towards the goal location.
        }
        \label{fig:GoalQs}
    \end{subfigure}%
    \hfill 
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/QvGP.pdf} 
        \caption{Model goal progress against the number of questions.
        DA and \acronymnormal{} generated \dia{}s make slower but consistent progress (ending below 25\% of total goal progress).
        }
        \label{fig:QvGP}
    \end{subfigure}
    \caption{Effectiveness of human \dia{}s (left) versus our models (right) at reaching the goal location.
    The slopes indicate the effectiveness of each \dia{} exchange in reaching the target.}
\end{figure*}
\setlength{\tabcolsep}{1.9pt}

\section{Analysis}
\label{sec:analysis}
We analyze the lexical diversity and effectiveness of generated questions by the \acronym{}.

\subsection{Lexical Diversity}
Both \acronym{} and Data Augmentation introduce new language by exploring and the environment and generating \dia{}s.
In the case of \acronym{}, an RL loss is used to update the models based on the most successful \dia{}.
Using Data Augmentation, the best generations are simply appended to the dataset for one epoch and weighted appropriately for standard, supervised training.
The augmentation strategy leads to small boost in BLEU performance and goal progress in several settings (Table~\ref{table:cvdn_results}), but the language appears to collapse to repetitive and generic interactions.
We see this manifest rather dramatically in Figure \ref{fig:lexdist}, where the DA is limited to only 22 lexical types.
In contrast, \acronym{} continues to produce over 500 unique lexical types, much closer to the nearly 900 used by humans.

\paragraph{Human Evaluation}
We collected human judgements comparing human dialogs with generated dialogs from the baseline and RMM agents on 254 randomly selected episodes from the \textit{unseen} validation set.
While RMM uses an RL objective to inform its language generation and achieves higher progress towards the goal in this setting (Table~\ref{table:cvdn_results}), it is rated as equally or more grammatical (57\%) and as equally or more fluent (60\%) than the baseline agent, suggesting that RMM’s generated language has not devolved into a “neuralese” to achieve better task performance.
Human dialogs were rated as equally or more grammatical and fluent than RMM (89\%/83\%) and the baseline (88\%/80\%).


\subsection{Effective Questions}
The \dia{} paradigm allows us to assess the efficacy of speech acts in accomplishing goals.
In a sense, the best question elicits the answer that maximizes the progress towards the goal room.
If agents are truly effective at modeling one other, we expect the number of \dia{} acts to be minimal.

Human conversations in CVDN always reach the goal location, and usually with only 3-4 questions, as shown in Figure~\ref{fig:GoalQs}.
We see that the relationship between questions and progress is roughly linear, excusing the occasional lost and confused human teams.
The final human-human question is often simply confirmation that navigation has arrived successfully to the goal room. 

In Figure \ref{fig:QvGP}, we plot \dia{}s for the Baseline, Data Augmentation, and \acronym{} agents against percent goal progress.
The \acronym{} consistently outperforms the other two agents in terms of goal progress for each \dia{} act. We see an  increase in progress for the first 10 to 15 questions before \acronym{} levels off.
By contrast, the Baseline and Data Augmentation agents exhibit shallower curves and fail to reach the same level of performance.


\subsection{Example \Dia{}}
While Figure \ref{fig:rmm} shows a cherry-picked \acronym{} trajectory from an \textit{unseen} validation house, Figure \ref{fig:val_unseen_trajectory} gives a lemon-picked \acronym{} trajectory.
We discuss the successes and failures of a lemon-picked---showcasing model failure---trajectory in Figure~\ref{fig:val_unseen_trajectory}.
As with all CVDN instances, there are multiple target object candidates (here, ``fire extinguisher'') but only one valid goal room.
Agents can become distracted by objects of the target instance in non-goal rooms.
When the \Or{} is shown the next few shortest path steps to communicate, those steps are towards the goal room.
As can be seen in Figure \ref{fig:val_unseen_trajectory}, the learned agents have difficulty in deciding when to stop and begin retracing their steps, and in this case never arrived to the correct goal room.

The learned models' generated language is of different levels of quality, with \acronym{} language much more coherent and verbose than Data Augmentation language.
Figure~\ref{fig:conversations} shows generated conversations along with the Goal Progress (GP) at each point when a question was asked.
Note that the generation procedure for all models use the same sampler, and they start training from the same checkpoint, so the relatively coherent nature of the \acronym{} as compared to the simple repetitiveness of the Data Augmentation is entirely due to the recursive calls and RL loss.
No model uses length penalties or other generation tricks to avoid degeneration.

\begin{figure}
\centering
\includegraphics[width=0.86\columnwidth]{images/MultiGoal.pdf}
\caption{Trajectories in an unseen environment attempting to find a target ``fire extinguisher.''
The red stop-sign is the goal room, while the black stop-sign is a non-goal room containing fire extinguishers.
The white trajectory is the human path from CVDN, black is the Baseline model, and green is our \acronym{}$_{N=3}$.}
\label{fig:val_unseen_trajectory}
\end{figure}


\begin{figure*}[ht!]
\centering
\begin{small}
\begin{tabular}{@{}l@{\hspace{5pt}}l@{\hspace{3pt}}p{7.6cm}@{\hspace{5pt}}l@{\hspace{3pt}}p{6.35cm}@{\hspace{5pt}}r@{}}
\toprule
 &  & Conversation & &&  GP\\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Human}} &\QI& Do I go in between the ropes to my right or straight forward? & \AI & straight forward through the next room  &0\\
& \QI& Should I proceed down the hall to the left of turn right? & \AI & head   down  the  hall to your  right into the  next room & 13.3 \\ 
& \QI& Should I go through the open doors that are the closest to me? & \AI & You are in  the  goal room & 29.1\\ 
\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{DA}} 
&\QI& should i go into the room? &\AI& you are in the goal room.& 5.7\\
&\QI& should i go into the room?&\AI& you are in the goal room.& 0.0\\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\acronym{}$_{N=3}$}} 
&\QI & should i head forward or bedroom the next hallway in front of me? &\AI & yes, all the way down the small hall.	&	4.0\\
&\QI & should i turn left here?  &\AI & head into the house, then you will find a doorway at the goal staircase. go through the doors before those two small exit chairs, about half way down the hall.	&	5.7\\
&\QI & lots of sink in this house, or wrong did. ok which way do i go &\AI & go down the hallway, take a left and go down the next hallway and up the stairs on the right.	&	8.8\\
\bottomrule
\end{tabular}
\end{small}
\caption{\Dia{} samples for Figure \ref{fig:val_unseen_trajectory} with corresponding Goal Progress -- see appendix for complete outputs.
}
\label{fig:conversations}
\end{figure*}


==> Dialogue Navigation/07-conclusions.tex <==
\section{Conclusions and Future Work}
We present a two-agent task paradigm for cooperative vision-and-\dia{} navigation (CVDN).
Existing work in vision-and-language navigation is largely limited to navigation only~(\ref{ch:act}), sometimes with limited additional instructions~(\ref{ch:act},\ref{ch:ans}).
By contrast, this work requires navigation~(\ref{ch:act}), question asking~(\ref{ch:que}), and question answering~(\ref{ch:ans}) components for learned, end-to-end \dia.
We find that simple speaker models 
are insufficient for the \dia{} setting, and demonstrate promising results from a recursive RL formulation with turn taking informed by theory of mind.

There are several limitations to the models presented in this paper.
We consider only agent-agent models, while the long-term goal of human-agent communication will require both human-in-the-loop training and evaluation.
Future work using \acronym{}-style modelling inspired by theory of mind will likely need to explicitly model the human interlocutor due to perceptual and communication differences~\cite{liu:aaai15}, rather than assuming the interlocutor can be modeled as a copy of oneself as in this paper.
Such modeling may incorporate world knowledge for richer notions of common ground, for example by explicitly detecting scene objects rather than using a fixed visual embedding~\cite{zhang:ijcai20}.
Additionally, we currently require the \Nr{} agent to ask questions after a fixed number of steps, while determining when to ask questions is a complex problem in itself~(\ref{ch:ask})~\cite{chi:aaai20}.
Furthermore, we use a fixed branching factor, while a dynamic branching factor in non-parametric learning setting can incorporate the uncertainty of the policy model. 

We hope this task paradigm will inspire future research on learning agent-agent, task-oriented communication with an eye towards human-agent cooperation and language-guided robots.


==> Dialogue Navigation/old/Old.tex <==
## 1



%The next step in embodied navigation is agents that not only follow instructions but also give them.  Vision-Language-Navigation (VLN) \cite{vln} provided a key benchmark for understanding the role that action taking has on language understanding.  However, a formulation, in which a human must correctly specify every action agents take in advance, is cumbersome at best and impossible in general.  Recent research \cite{help_anna} has started to enrich the instruction paradigm by only requiring the human to provide a high-level goal, while the agent can ask for help if it gets lost.  In this work, we close the loop by leveraging the Cooperative Vision-Dialogue Navigation dataset introduced in \cite{cvdn} to train a full dialogue system, in which embodied visual agents follow instructions, ask for clarifications, and provide guidance on where to move next.  Every interaction is communicated in natural language and our system leverages the same Matterport house environment \cite{matterport}. The strength of a dialogue based agent is that long trajectories can be traversed without dramatically increasing the burden on the human.  Specifically, our models will be required to cover \YBi{X} meters around homes where the original VLN agents only learned to navigate \YBi{Y}.

%Relatedly, negotiation \cite{cao2018emergent} can help facilitate the creation of emergent communication.  
%Key to all of these approaches is the need to model the listener via Theory-of-Mind \cite{theory_of_mind_child}.  A good question will elicit an informative answer and an informative answer will help the agent achieve their goal.  In theory, this recursion could execute indefinitely.  In practice, humans maximize locally while moving the conversation globally.  To formalize this intuition, we introduce a \approach{} (\acronym) which spawns instances of itself to explore the space of conversations and actions.  this leads now only to better agents but also more natural language.


%Vision-Dialogue 
%Current problems with CVDN task: 
%
%R2R Instructions are given step-by-step so if follower makes a single wrong turn, instructions become useless. 
%
%Insufficient exploration of environment 
%
%No follower feedback (All instructions are generated before any actions are taken).
%\dots

%Where is the field right now ?
%What we are doing
%Why
%- paragraph 2 -
%How
%- prev work if strongly relevant
%What findings
%- paragraph 3 -
%- What results

%- Contributions: New task, new dataset, new results
%-- General Enough the community can use
%Should be able to see what comes next


## 3
%Our task asks, given a navigator $\mathcal{N}$, a questioner $\mathcal{Q}$, and an oracle $\mathcal{O}$, can an agent successfully traverse a house by engaging in a natural language conversation.  The $\mathcal{N}$avigator takes instructions as input and produces actions to move throughout the house.  We use the original primitive action space introduced by the original VLN task to move through the environment. This requires the agent to actually understand perspective as instructions might include ``turn around." This is in contrast to recent work focusing on panoramic perspectives that assume the agent can see in all directions.    Next, when the agent stops walking, the $\mathcal{Q}$uestioner asks for clarification about the next actions to take.  In the worst case the agent might simply be lost and ask for help, but in general, these questions contain specific requests that reference the trajectory (e.g. ``should I go back to the room I just passed or continue on?").  Finally, the $\mathcal{O}$racle is a third trained agent which answers questions by viewing the near (five step) future of a shortest path towards the goal.  Again, note that a naive $\mathcal{O}$racle might simply provide step by step instructions (e.g. forward, forward, right, ...), but these responses are unnatural and would not address the question asked by the $\mathcal{Q}$uestioner.  In practice, $\mathcal{N}, \mathcal{Q}$, and $\mathcal{O}$ are implemented as sequence-to-sequence based neural models equipped with visual attention.

%Specifically, algorithm \ref{alg:dialogue-navigation} illustrates Dialogue Navigation.


%\subsection{Datasets}
% We initialize our models using two available datasets: 1. Vision-Language-Navigation and 2. The Navigation Dialogue History (NDH) formulation of the CVDN dataset.  Even though VLN differs in its goals, it provides a large in domain dataset for grounded visual language.  This allows us to pretrain $\mathcal{Q}$ and $\mathcal{O}$ to produce relevant natural language sentences.  Next, we can fine-tune our models on the data from NDH.  NDH was introduced as a task by The Cooperative Vision and Dialogue Navigation Dataset (CVDN) where dialogue histories are collapsed to form a long input instruction similar to the VLN formulation.  

%CVDN is comprised of 2050 dialogues between two human speaker-follower players where the goal is for the follower to reach the closest location with the target object as quickly as possible. Each dialogue is a sequence of question-answer interactions covering nearly 7,000 different trajectories in 83 Matterport indoor environments. The goal of the conversation is to find a target location which is specified up front in natural language (e.g. a fire-extinguisher).  In CVDN, all targets are both ambiguous and underspecified to force dialogue and overcome basic structural priors (e.g. toilets are in bathrooms). In practice, this means that no step-by-step instructions are provided or immediately deducible from the start without asking for help. NDH refers to the task of treating the dialogue history as a static set of instructions (a la VLN) and several recent papers have focused on performing this task \cite{xin,cvdn}.

%Our aims are more ambitious, we not only want an agent to understand a static dialogue but to generate its own.  To do this, we will train our models $\mathcal{N}, \mathcal{Q}$, and $\mathcal{O}$ on their respective roles in the data, but all gold information will be discarded during evaluation.  To ensure we maintain a fair comparison for upper-bound human performance, we will evaluate with the same house scans \textit{S}, starting position starting position $p_0$, and the target object $t_o$.  In this way we can directly compare the quality of our dialogues quantitatively (e.g. how far are we from goal and how many questions did we require?).  We analyze this in detail in Section \ref{sec:analysis}.
%CVDN identifies as targets a set of 81 different objects that are common and appear 2 or more times in at least 5 different Matterport indoor environments. The initial dialogue prompts include the house scan \textit{S}, the starting position $p_0$, and the target object $t_o$. 


%\subsection{Evaluation Metrics}
%For evaluation of the agent, we use the goal progress which refers to the amount of distance in meters covered from the starting position to the goal location along the shortest path. As for the speaker, we use the BLEU score between the generated dialogue history and the ground truth human dialogue for the trajectory. It should be noted that due to noise in the data like wrong human instructions, it is not necessarily always desirable to get a BLEU score of 1.0 at the expense of lower agent performance.



## 4 

%\subsection{Implementation details}
%As previously done in vision language navigation\cite{vln}, we use as image features $\Tilde{f}$ the output from the last convolutional layer of ResNet\cite{resnet} trained on ImageNet\cite{imagenet}. 
%These image features are not changed during training or testing.

%\subsubsection{Pre-training NDH task on CVDN.} 
%Leveraging results from meta-learning\cite{maml} where meta-learning leads to faster adaptation of deep networks, we pre-train the NDH task on the CVDN dataset.
%For pre-training, the agent is allowed to see the entire dialogue history from the start. However, no new questions or answers are generated while the agent is training. 
%Figure ~\ref{fig:action_decoder} illustrates how action decoding is done at each time step. Before the agent is placed in the environment,
%the entire dialogue history is feed in to an LSTM encoder with a word embedding size of 256,
%a hidden size of 512, training dropout ratio of 50\%, and max input length of 160 tokens. 
%The LSTM encoder outputs a hidden state $\Tilde{h}_{t-1}$ and a context $[u_1,...,u_j]$ where each $u_j$ corresponds to an encoded
%instruction token. The context $[u_1,...,u_j]$ is constant because in the NDH task, the instructions do not change. Then at each time step, the decoder takes in the previous action $\Tilde{a}_{t-1}$,
%which initially is \textit{start}, the current panorama features $\Tilde{f}_t$, and the k navigable viewpoint features $\Tilde{g}_{t,k}$. The decoder is an attentive LSTM Decoder as shown in figure \ref{fig:action_decoder}. Action embedding size and target embedding size are 32. 



% \subsection{The Navigation from Dialogue History Task (NDH)}

% as shown in equation \ref{eq:cross_entropy}.  

% \begin{align}
%   CE(X,Y) & = -\sum_{i}^{C} y_i \ log \ (\textbf{Softmax}(x)_i) \label{eq:cross_entropy}
% \end{align}
%\subsection{The Collaborative Vision Dialogue Navigation Task}
%Traditionally, in Vision-Language Navigation, the agent has full access to instructions from start to finish. 
%However, having access to these instructions is not sufficient. 
%Agents that get lost along the way may suffer from having misaligned instructions.
%Instead, a more realistic scenario for Collaborative Vision Dialogue Navigation is to allow the agent 
%to ask for help in the form of a question and get a response in the form of an answer as the agent
%acts upon its environment. This new approach is the Collaborative Vision Dialogue Navigation gameplay 
%illustrated below. \\
%
%%\begin{wrapfigure}[5]{l}{\linewidth}
%%\centering
%%\vspace{-25pt}
%%\caption{Illustration of gameplay}
%%\vspace{-5pt}
%%\includegraphics[width=\linewidth]{images/gameplay.JPG}
%%\label{fig:gameplay}
%%\end{wrapfigure}
%
%Under this formulation, the agent starts only with egocentric 
%knowledge of the objects in front of it and the target it needs to reach. 
%Its only actions are to move forward, turn up, down, left, or right. 
%At any point in time, the agent may recognize it got lost and ask a question.
%The question is generated by paying attention to the images at the viewpoint where the agent decided to ask the question.
%In order to reply to that question, the speaker looks a the next five steps in the shortest path to the goal
% then, by attending to the images along this path, samples word-by-word to generate a text answer.
% With the new question-answer pair, the agent updates its context to predict the next action.
% The agent may choose to save its dialogue history in which case the entire previous dialogue history along
% with the new question and answer are used to update the context.
% Finally, the rollout ends when the agent decides to stop. 

%We generate additional data by sampling from a navigator model and allowing it to get lost.
%To augment the data, during training, each regular agent rollout also generates trial runs with different actions sampled based on the sampling or action-choosing technique being used. Also full dialog histories are generated out of these trial runs. One of the trial runs is the one where instead of sampling, the agent selects the argmax action from its predicted logits. This ensures that the best trial run will perform no worse than the argmax. Once these trial runs are generated, the one with the greatest goal progress is selected to do training on where the generated data is treated as ground truth and trained on.

%As another way to augment the data, we leverage the technique of random start where the agent can start anywhere in the simulator as long as the starting viewpoint has at least one viable path to the goal. In order to guarantee that the new starting position can reach the goal we introduce a \textit{Jitter} parameter that determines how far is the new starting position expected to be from the original initial position. For instance, a \textit{Jitter} of 1 indicates that the new starting position is a neighbor of the original starting position.


When the agent asks a question, words are sampled word-by-word but instead of only generating a single question, we generate $N$ candidate questions.
Then, when generating answers for each candidate question, we generate $N$ candidate answers. This produces a total of $N^2$ 
different candidate question-answer pairs. In order to choose which of these pairs is expected to get the agent closest to the end goal, 
an \acronymnormal\ is run for each pair. Inside the \acronymnormal\ a previous version of the agent is run to completion.
As it runs, this \acronymnormal\ agent may potentially ask a question which would trigger a recursive call to a new \acronymnormal .\
This recursive process continues until the \acronymnormal\ agent decides to stop. To prevent a potentially infinite number of \acronymnormal s,
the branching factor may change to prevent going above a certain computational limit. 
At any given point in time, there are at most $N^2$ different candidate question-answer pairs being mentally run. 
This is achieved by decreasing the branching factor from $N$ to 1 on subsequent recursive calls. 
Once all the $N^2$ candidates decide to stop, the model picks the answer for which the \acronymnormal\ agent got closest to the goal.
This answer is then returned to the original agent as the best answer. The original agent updates its saved dialogue history and continues it rollout.
A new question may be asked which would once again trigger the creation of \acronymnormal s.\ 
This continues until the original agent decides to finally stop. \\
By exposing the goal progress metric to the speaker, the \acronymnormal\ also allows the speaker to leverage Reinforcement Learning techniques.
This is an novel approach with much to be explored. 
In particular, this paper shows the effects of training the speaker with the cross entropy loss between the human and the generated dialogues added to the best-answer \acronymnormal\ RL agent loss.


\subsection{Experiments}

\subsubsection{CVDN Gameplay Baseline} In the CVDN task, the only initial input is the target, 
so after pre-training with the NDH task, we follow the same action decoding scheme as in figure \ref{fig:action_decoder}.
However, the context $[u_1,...,u_j]$ is no longer fixed. The dialogue history starts as only the target but increases 
as more questions are asked and answered. The hidden state $\Tilde{h}_{t-1}$ is not cleared out on each context change.
We use a batch size of 10 and train for 20000 iterations.
Also, since the average number of steps between questions is 4.46, we use 4 as the number of steps between each
question and leave the exploration on when to ask a question and topic of future work.
Furthermore, since questions are generated and answered as the agent is interacting with the environment it is also possible to train the 
speaker as it generates new responses. The baseline of CVDN gameplay; however, does not train the speaker beyond the pre-training.
The Data Augmentation and \acronymnormal\ models do train the question and answer generation system. \\
Figure \ref{fig:instruction_decoder} illustrates how instruction decoding is done. It should be noted that the model that generates questions is the same as the model that generates answers, the only difference between the two is that when generating questions, we start the sequence with the \textit{$<$NAV$>$} tag and use only the current viewpoint as input features whereas to generate an answer we start the sequence with the  \textit{$<$ORA$>$} tag and use the visual features from the next 5 viewpoints along the shortest path to the goal.

% \begin{figure}
%\centering
%\includegraphics[width=\linewidth]{images/instruction_decoder.JPG}
%\caption{Illustration of Seq2Seq instruction decoding}
%\label{fig:instruction_decoder}
%\end{figure}

%\subsubsection{Data Augmentation} 
%In the data augmentation model, on each iteration we do teacher forcing as in the original CVDN Baseline formulation but with speaker training and filter from 3 trials runs for the one that had a final distance closest to the goal. On each trial run, we output to a log file the trajectory and generated dialogue history. One of the trial runs uses the argmax from the predicted action logits while the rest sample for the next action. In practice, each trial run has a standard deviation of about 3 meters. From the log file we filter for the run that got closest to the goal and train on the output from this best run adding $\lambda$\% of this augmented loss to the total loss. The analysis section has an exploration of this $\lambda$ parameter but, in short, we found $\lambda=0.1$ to work best. We find that without including the argmax as a trial run and with no $\lambda$ parameter, the speaker quickly starts to deviate away from English language leading to worse performance. 
%\subsubsection{\acronymnormal} 
%As the name implies, \acronymnormal\ is implemented recursively. 
%On every four time steps, the agent generates 3 sampled word-by-word questions each of which leads to 3 sampled candidate answers for a total of 9 question-answer pairs. For each question-answer pair, the speaker loads a previous instance of the agent as a Mental Model with the  question-answer pair concatenated to its dialogue history. As it rolls out, after every 4 steps, the Mental Model agent may also ask for a question at which point another mental model agent is run with a newly sampled question-answer pair concatenated to its dialogue history but with a single candidate instead of 9. This interaction of going deeper and deeper into the recursive stack continues until the last-layer Mental Model agent decides to stop or reaches the maximum limit of 80 episodes. Once at the last layer, the top-most mental model agent returns its goal progress which propagates recursively all the way back to the first recursive call. With the goal progresses from the 9 Mental Models, the speaker can pick the answer and question which led to the most goal progress. The original agent, then receives the new question-answer pair, concatenates it to its dialogue history and continues its rollout once again asking for help at the next 4 time steps which will lead to 9 new Mental Models and so on until the original agent decides to stop or runs out of episodes.
%
%\subsection{Action Probabilities}
%In order to select the best question-answer pair from the candidates on each mental model run, during evaluation instead of using the Goal Progress, the agent leverages the average of its last action probabilities as a signal. This way, the model picks the question-answer pair for which the respective mental model was most confident out of all the candidates.


## 5

% \subsection{Analysis on Data Augmentation}
% \subsubsection{Contribution of Data Augmentation}
% Fig.~\ref{fig:gp_vs_iter} for Goal Progress vs iteration for different lambdas of data augmentation
% % \subsubsection{Temperature Sampling}
% % Fig.~\ref{fig:temperature} illustrates Goal Progress vs number of Data augmentation teacher forcing rounds
% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{images/gp_vs_iter.JPG}
% \caption{Data Augmentation Goal Progress vs  Iteration}
% \label{fig:gp_vs_iter}
% \end{figure}
% 
% % \begin{figure}
% % \centering
% % \includegraphics[width=\linewidth]{images/gp_vs_aug.JPG}
% % \caption{Goal Progress vs Data Augmentation Rounds}
% % \label{fig:temperature}
% % \end{figure}
% \subsubsection{Random Start}
% \subsection{Analysis on \acronymnormal}




%\setlength{\tabcolsep}{4pt}
%\begin{table}
%\centering
%\caption{Gameplay results on NDH}
%\label{table:results}
%\begin{small}
%\begin{tabular}{lclclclclclc}
%\hline\noalign{\smallskip}
%\textbf{Fold} & \textbf{Model} & \textbf{Input} & \multicolumn{2}{c}{\textbf{Generated}} & \textbf{Goal Progress(m)} & \textbf{BLEU} \\
%  &   & $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$&$\uparrow$&$\uparrow$\\
%\hline \noalign{\smallskip}
%\multirow{16}{*}{\rotatebox[origin=c]{90}{Val Seen}}  &  \multirow{4}{*}{Baseline} &\multicolumn{3}{c}{Shortest Path Agent}& 9.359 & 1.0\\
%& & \ding{51} & & & 1.733 & None\\
%& & \ding{51} & \ding{51} & & 1.688 & 0.0383\\
%& & \ding{51} & \ding{51} & \ding{51} & 1.662 & 0.0386 \\
%\cline{2-7}& \multirow{3}{*}{Data Aug} & \ding{51} & & & 2.632 & None\\
%& & \ding{51} & \ding{51} & & 2.519 & 0.0298\\
%& & \ding{51} & \ding{51} & \ding{51} & 1.358 & 0.0328\\
%\cline{2-7} \noalign{\smallskip} & Data Aug & \ding{51} &  & & - & None\\
%& + & \ding{51} & \ding{51} & & - & -\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \multirow{3}{*}{\acronymnormal} & \ding{51} &  &  & - & None\\
%& & \ding{51} & \ding{51} & & - & -\\
%& & \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \acronymnormal & \ding{51} &  &  & - & None \\
%& + & \ding{51} & \ding{51} & & - & -\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\hline
%\noalign{\smallskip}
%\multirow{16}{*}{\rotatebox[origin=c]{90}{Val Unseen}}  &  \multirow{4}{*}{Baseline} &\multicolumn{3}{c}{Shortest Path Agent}& 9.831 & 1.0\\
%& & \ding{51} & & & 0.184 & None\\
%& & \ding{51} & \ding{51} & & 0.216 & 0.0382\\
%& & \ding{51} & \ding{51} & \ding{51} & 0.398 & 0.0365\\
%\cline{2-7}& \multirow{3}{*}{Data Aug} & \ding{51} & & & 0.387 & None\\
%& & \ding{51} & \ding{51} & & 0.350 & 0.0419\\
%& & \ding{51} & \ding{51} & \ding{51} & \textbf{0.484} & \textbf{0.0423}\\
%\cline{2-7}\noalign{\smallskip} & Data Aug & \ding{51} &  &  & - & None\\
%& + & \ding{51} & \ding{51} & & - & -\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \multirow{3}{*}{\acronymnormal} & \ding{51} &  &  & - & None\\
%& & \ding{51} & \ding{51} & & - & -\\
%& & \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \acronymnormal & \ding{51} &  &  & - & -\\
%& + & \ding{51} & \ding{51} & & - & None\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\hline
%\end{tabular}
%\end{small}
%\end{table}


## Appendix

% \setlength{\tabcolsep}{4pt}
% \begin{table}
% \centering
% \caption{Generated Conversations}
% \label{table:conversations}
% \begin{small}
% \begin{tabular}{lcp{10.6cm}}
% \toprule
%  & & Conversation \\
% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Human}} & Q:& Should I head into the room with the table ?\\
% & A:& head into the room with the table, turn to the left and head down the hall to the stairs \\ 
% \midrule
% \multirow{11}{*}{\rotatebox[origin=c]{90}{Baseline}} & Q:& i am lost . where should i go next ? \\
% & A:& turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go into the bedroom . go through the door to your right . go through the door to your right , move forward forward on your right .\\
% & Q:& i am lost . where should i go next ? \\
% & A:& exit the room . turn right and go through the door on the right .  go through the first door on your right .\\
% & Q:& i am lost . where should i go next ?\\
% & A:& go to the right . go to the stairs . go up the stairs . yes , go forward forward on the right .\\
% \midrule
% \multirow{9}{*}{\rotatebox[origin=c]{90}{Data Augmentation}} & Q:& i am lost . where should i go next ?\\
% & A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
% & Q:& i am lost . where should i go next ?\\
% & A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
% & Q:& i am lost . where should i go next ?\\
% & A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
% \midrule
% \multirow{11}{*}{\rotatebox[origin=c]{90}{\acronymnormal}} & Q:& this is not the room . should i go through the door , the open doorway , or up the stairs ?\\
% & A:& go out the open door in front of you . you should see a dining table to your right as you exit \\
% & Q:& should i go toward the green door , the open doorway , or up the stairs ? \\
% & A:& you will see a few stairs to your right as you exit \\
% & Q:& where should i go from here ? \\
% & A:& left past the plant . \\
% & Q:& i am in the bathroom at the bottom of the stairs .  should i move or toward the bedroom ? \\
% & A:& left and then right in the room that will be on the desk \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{table}
% \setlength{\tabcolsep}{1.4pt}

\subsubsection{Pre-training on R2R and NDH}

Table~\ref{table:pretrain} shows results from pre-training of agent and speaker
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Pre-training results on NDH}
\label{table:pretrain}
\begin{tabular}{lcccccc}
\hline\noalign{\smallskip}
\textbf{Fold} & \textbf{Task(s) Trained} & \multicolumn{3}{c}{\textbf{Seq-2-Seq Input}} & \textbf{Goal Progress} & \textbf{BLEU} \\
  &   & $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$&$\uparrow$&$\uparrow$\\
\hline \noalign{\smallskip}
\multirow{4}{*}{\rotatebox[origin=c]{90}{Val Seen}} &   &\multicolumn{3}{c}{Shortest Path Agent}& 9.359 & 1.0\\
 & NDH  & \ding{51} & \ding{51} & \ding{51} & 5.92  & None\\
 \cline{2-7} \noalign{\smallskip} & NDH follower  & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{5.261} & \multirow{2}{*}{\textbf{0.0009}}\\
  & R2R + NDH speaker & & & &\\
\hline
\noalign{\smallskip}
\multirow{2}{*}{\rotatebox[origin=c]{90}{Val Unseen}}  &   &\multicolumn{3}{c}{Shortest Path Agent}& 9.831 & 1.0\\
& NDH   & \ding{51} & \ding{51} & \ding{51} & 2.10  & None \\
\cline{2-7} \noalign{\smallskip} & NDH follower  & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{2.018} & \multirow{2}{*}{\textbf{0.0007}}\\
  & R2R + NDH speaker & & & &\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.9pt}




Table~\ref{table:cvdn_rl} shows follower RL vs full RL results on CVDN
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Follower RL vs full RL results on CVDN}
\label{table:cvdn_rl}
\begin{tabular}{cccccccc}
\hline\noalign{\smallskip}
\multicolumn{2}{c}{\textbf{Fold}} &  \multicolumn{2}{c}{\textbf{Generated}} &
\multicolumn{2}{c}{\textbf{RL Trained}} & \textbf{Goal Progress} & \textbf{BLEU} \\
  & & $Q_i;A_i$& $Q_{i-1};A_{i-1}$& A2C& Speaker &$\uparrow$&$\uparrow$\\
\hline \noalign{\smallskip}
\multirow{2}{*}{Val Seen} &  & \ding{51} & \ding{51} & \ding{51} & & - & - \\
  &   & \ding{51} & \ding{51} & \ding{51} & \ding{51} & - & -\\

\hline
\noalign{\smallskip}
\multirow{2}{*}{Val Unseen}  &  & \ding{51} & \ding{51} & \ding{51} &  & - & -\\ 
  &   & \ding{51} & \ding{51} & \ding{51} & \ding{51} & - & - \\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.9pt}

\setlength{\tabcolsep}{4pt}
\begin{table}
\centering
\caption{Gameplay results on NDH}
\label{table:results}
\begin{small}
\begin{tabular}{llcccccc}
\toprule
 & \textbf{Model} & \multicolumn{3}{c}{\textbf{Goal Progress (m) $\uparrow$}} & \multicolumn{3}{c}{\textbf{\textbf{BLEU} $\uparrow$}} \\
  &   & $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$& $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$\\
\hline \noalign{\smallskip}
\multirow{6}{*}{\rotatebox[origin=c]{90}{Val Seen}}  &  
  Shortest Path &       &       & 9.359 &      &        & --\\
& Baseline      & - & - & - & -- & - & -\\
& DA      & - & - & - & -- & - & - \\
& DA + RS &       &       &       & -- &        & \\
\cline{2-8}   
& \acronymnormal        &       &       &       & -- &     &\\
& \acronymnormal{} + RS &       &       &       & -- &     & \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{Val Unseen}}  &  
  Shortest Path &       &       & 9.831 &      &        & --\\
& Baseline      & - & - & - & -- & - & -\\
& DA            & - & - & - & -- & - & - \\
& DA + RS       &       &       &       & --   &        & \\
\cline{2-8}   
& \acronymnormal        &       &       &       & -- &     &\\
& \acronymnormal{} + RS &       &       &       & -- &     & \\
\bottomrule
\end{tabular}
\end{small}
\end{table}
\setlength{\tabcolsep}{1.9pt}



\begin{align}
  CE(X,Y) & = -\sum_{i}^{C} y_i \ log \ (\textbf{Softmax}(x)_i) \label{eq:c_e}\\
  & where \quad \textbf{Softmax}(x)_i = \frac{e^{x_i}}{\sum_{j}^{C}e^{x_j}}
\end{align}


\setlength{\tabcolsep}{4pt}
\begin{table}
\centering
\caption{Generated Conversations}
\label{table:prev_conversations}
\begin{small}
\begin{tabular}{lcp{10.6cm}}
\toprule
 & & Conversation \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Human}} & Q:& Should I head into the room with the table ?\\
& A:& head into the room with the table, turn to the left and head down the hall to the stairs \\ 
\midrule
\multirow{11}{*}{\rotatebox[origin=c]{90}{Baseline}} & Q:& i am lost . where should i go next ? \\
& A:& turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go into the bedroom . go through the door to your right . go through the door to your right , move forward forward on your right .\\
& Q:& i am lost . where should i go next ? \\
& A:& exit the room . turn right and go through the door on the right .  go through the first door on your right .\\
& Q:& i am lost . where should i go next ?\\
& A:& go to the right . go to the stairs . go up the stairs . yes , go forward forward on the right .\\
\midrule
\multirow{9}{*}{\rotatebox[origin=c]{90}{Data Augmentation}} & Q:& i am lost . where should i go next ?\\
& A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
& Q:& i am lost . where should i go next ?\\
& A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
& Q:& i am lost . where should i go next ?\\
& A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
\midrule
\multirow{11}{*}{\rotatebox[origin=c]{90}{\acronymnormal}} & Q:& this is not the room . should i go through the door , the open doorway , or up the stairs ?\\
& A:& go out the open door in front of you . you should see a dining table to your right as you exit \\
& Q:& should i go toward the green door , the open doorway , or up the stairs ? \\
& A:& you will see a few stairs to your right as you exit \\
& Q:& where should i go from here ? \\
& A:& left past the plant . \\
& Q:& i am in the bathroom at the bottom of the stairs .  should i move or toward the bedroom ? \\
& A:& left and then right in the room that will be on the desk \\
\bottomrule
\end{tabular}
\end{small}
\end{table}
\setlength{\tabcolsep}{1.4pt}



### Old 


%% %\setlength{\tabcolsep}{4pt}
%% \begin{table*}
%% \centering
%% \begin{small}
%% \begin{tabular}{ll@{\hspace{2em}}cc@{\hspace{2.5em}}ac@{\hspace{2.5em}}ca}
%%  & \textbf{Model} & \multicolumn{4}{c}{\textbf{Goal Progress (m) $\uparrow$}} & \multicolumn{2}{c}{\textbf{\textbf{BLEU} $\uparrow$}} \\
%% \toprule
%%   &   & $t_0$& $QA_i$& $QA_{i-1:0}$& \begin{scriptsize}\begin{tabular}{@{}c@{}}+\! Oracle\\Stopping\end{tabular}\end{scriptsize} & $QA_i$& $QA_{i-1:0}$\\
%%   \midrule
%% \multirow{5}{*}{\rotatebox[origin=c]{90}{Val Seen}}  
%% & Baseline                       &\textbf{20.11}& 10.52      & \Be{14.96}     & \textbf{22.9} & 0.9    & 0.8     \\
%% & Data Augmentation                      & 20.11    & 10.51      & 10.04     & 14.2 & 1.3    & 1.3     \\
%% %& DA + RS                       &\Be{20.48}& 10.80      & \Be{15.01}&      & 1.3    & 0.3     \\
%% & \acronym$_{N=1}$               &18.73     & 10.02      & 13.27     & 20.4 & 3.3    & 3.0     \\
%% %& \acronym$_{N=1}$ +RS          &19.82     & 10.57      & 11.51     & --   &\Be{3.5}& 3.1     \\
%% & \acronym$_{N=3}$ +AP           &18.90     & \textbf{11.54} & 13.97 & 16.8 &\textbf{3.4}&\Be{3.6}\\
%% %\cline{2-8}   
%% %& Perfect \acronym$_{N=3}$      &18.90     & 7.42       & 11.00     & -- & 3.4    & 3.5 \\
%% %& Perfect \acronym$_{N=3}$ + RS &15.64     & 9.48       & 11.61     & -- & 3.5    & 3.3\\
%% &  Shortest Path                 & \multicolumn{4}{@{}c}{----------- 32.79 ----------- }    &   & \cellcolor{white}\\
%% \midrule
%% \midrule
%% \multirow{5}{*}{\rotatebox[origin=c]{90}{Val Unseen}}    
%% & Baseline                           & 6.78     & 4.67      & \PZ4.55      & 6.34& 0.5  & 0.5\\
%% & Data Augmentation                                 & 6.78     & 5.47      & \PZ4.38      & 6.52& 1.3  & 1.1\\
%% %& DA + RS                           & 4.408    & \Be{6.15} & \PZ3.07      & --  & 1.2  & 0.3\\
%% & \acronym$_{N=1}$                   & 6.10     &\textbf{6.09}  & \PZ5.11      & 5.95 & 2.6  & 2.8\\
%% %& \acronym$_{N=1}$ +RS              & 5.838    & 5.488     & \PZ6.24      & --  & 2.9  & 2.7\\
%% & \acronym$_{N=3}$ +AP               &\textbf{7.26} & 5.53      & \PZ\Be{5.61} &\textbf{8.87} &\textbf{2.9}&\Be{2.9}\\
%% %\cline{2-8}          
%% %& Data Aug. \hspace{8pt} + O Stop   &          &           & \PZ6.52      &     &      &      \\
%% %& \acronym$_{N=3}$ +AP + O Stop     &          &           & \PZ8.87      &     &      &      \\
%% %& \acronym$_{N=3}$ + O branch       &          &           & \PZ8.16      & --  & 2.9  & 2.9\\
%% %& \acronym$_{N=3}$ + O branch       &   7.26   & 8.11      & \PZ8.16      & --  & 2.9  & 2.9\\
%% %& Perfect \acronym$_{N=3}$ + RS     &   6.098  & 7.563     & \PZ7.01      & --  & 2.8  & 2.9\\
%% & Shortest Path                     & \multicolumn{4}{@{}c}{----------- 29.32 ------------}                & & \cellcolor{white} \\
%% \bottomrule
%% \end{tabular}
%% \end{small}
%% \caption{Gameplay results on CVDN -- All results evaluated when agent voluntarily stops or at 80 steps.}
%% \label{table:cvdn_results}
%% \end{table*}



%\paragraph{Initial Models}
%In Table \ref{table:pretrain_cvdn} we see that this initialization works well on seen navigation environments.  In contrast, while pretraining does help our final speaker models, note that the generation task for NDH is substantially more difficult than seen in the literature for VLN.  This is likely due to longer sequences and co-reference.

% \begin{table}
% \begin{small}
% \begin{center}
% \begin{tabular}{lccccc}
% \hline\noalign{\smallskip}
% \textbf{Fold} & & \textbf{Goal Progress}$\uparrow$ & \textbf{BLEU}$\uparrow$ \\
% \hline \noalign{\smallskip}
% \multirow{2}{*}{Seen}  & Gold  & 32.789 & -- \\
%                        & Pretraining & 20.840  & 0.20\\
% \midrule
% \noalign{\smallskip}
% \multirow{2}{*}{Unseen}  & Gold & 29.321 & -- \\
%                          & Pretraining & 6.550  & 0.19 \\
% 
% \hline
% \end{tabular}
% \end{center}
% \end{small}
% \caption{Performance of initial models on navigating from and generating full dialogues during pretraining.}
% \label{table:pretrain_cvdn}
% \end{table}



%\paragraph{Stopping Criteria}
%Under this implementation, the agent can only stop when it either voluntarily decides to predict the STOP action or when it runs out of steps. Previous work \cite{cvdn}  has used a max length of 80 steps; therefore, in this paper we also have this limit. It should be noted that because of this restriction results may not be as optimal as in the case when the agent has a known per-trajectory maximum number of steps.   


%# Seen      CSV     Homero
%baseline = [19.85, 10.06]
%dataaugm = [10.09, 10.00]
%rmmn1    = [15.53, 11.00]
%rmmn3    = [13.81, 14.13]
%print(ave(baseline), ave(dataaugm), ave(rmmn1), ave(rmmn3))
% 14.96 10.04 13.27 13.97
%
%# Unseen    CSV   Homero
%baseline = [3.44, 5.67]
%dataaugm = [4.19, 4.58]
%rmmn1    = [3.94, 6.28]
%rmmn3    = [5.34, 5.88]
%print(ave(baseline), ave(dataaugm), ave(rmmn1), ave(rmmn3))
%  4.55  4.38  5.11  5.61



==> old/Old.tex <==
## 1



%The next step in embodied navigation is agents that not only follow instructions but also give them.  Vision-Language-Navigation (VLN) \cite{vln} provided a key benchmark for understanding the role that action taking has on language understanding.  However, a formulation, in which a human must correctly specify every action agents take in advance, is cumbersome at best and impossible in general.  Recent research \cite{help_anna} has started to enrich the instruction paradigm by only requiring the human to provide a high-level goal, while the agent can ask for help if it gets lost.  In this work, we close the loop by leveraging the Cooperative Vision-Dialogue Navigation dataset introduced in \cite{cvdn} to train a full dialogue system, in which embodied visual agents follow instructions, ask for clarifications, and provide guidance on where to move next.  Every interaction is communicated in natural language and our system leverages the same Matterport house environment \cite{matterport}. The strength of a dialogue based agent is that long trajectories can be traversed without dramatically increasing the burden on the human.  Specifically, our models will be required to cover \YBi{X} meters around homes where the original VLN agents only learned to navigate \YBi{Y}.

%Relatedly, negotiation \cite{cao2018emergent} can help facilitate the creation of emergent communication.  
%Key to all of these approaches is the need to model the listener via Theory-of-Mind \cite{theory_of_mind_child}.  A good question will elicit an informative answer and an informative answer will help the agent achieve their goal.  In theory, this recursion could execute indefinitely.  In practice, humans maximize locally while moving the conversation globally.  To formalize this intuition, we introduce a \approach{} (\acronym) which spawns instances of itself to explore the space of conversations and actions.  this leads now only to better agents but also more natural language.


%Vision-Dialogue 
%Current problems with CVDN task: 
%
%R2R Instructions are given step-by-step so if follower makes a single wrong turn, instructions become useless. 
%
%Insufficient exploration of environment 
%
%No follower feedback (All instructions are generated before any actions are taken).
%\dots

%Where is the field right now ?
%What we are doing
%Why
%- paragraph 2 -
%How
%- prev work if strongly relevant
%What findings
%- paragraph 3 -
%- What results

%- Contributions: New task, new dataset, new results
%-- General Enough the community can use
%Should be able to see what comes next


## 3
%Our task asks, given a navigator $\mathcal{N}$, a questioner $\mathcal{Q}$, and an oracle $\mathcal{O}$, can an agent successfully traverse a house by engaging in a natural language conversation.  The $\mathcal{N}$avigator takes instructions as input and produces actions to move throughout the house.  We use the original primitive action space introduced by the original VLN task to move through the environment. This requires the agent to actually understand perspective as instructions might include ``turn around." This is in contrast to recent work focusing on panoramic perspectives that assume the agent can see in all directions.    Next, when the agent stops walking, the $\mathcal{Q}$uestioner asks for clarification about the next actions to take.  In the worst case the agent might simply be lost and ask for help, but in general, these questions contain specific requests that reference the trajectory (e.g. ``should I go back to the room I just passed or continue on?").  Finally, the $\mathcal{O}$racle is a third trained agent which answers questions by viewing the near (five step) future of a shortest path towards the goal.  Again, note that a naive $\mathcal{O}$racle might simply provide step by step instructions (e.g. forward, forward, right, ...), but these responses are unnatural and would not address the question asked by the $\mathcal{Q}$uestioner.  In practice, $\mathcal{N}, \mathcal{Q}$, and $\mathcal{O}$ are implemented as sequence-to-sequence based neural models equipped with visual attention.

%Specifically, algorithm \ref{alg:dialogue-navigation} illustrates Dialogue Navigation.


%\subsection{Datasets}
% We initialize our models using two available datasets: 1. Vision-Language-Navigation and 2. The Navigation Dialogue History (NDH) formulation of the CVDN dataset.  Even though VLN differs in its goals, it provides a large in domain dataset for grounded visual language.  This allows us to pretrain $\mathcal{Q}$ and $\mathcal{O}$ to produce relevant natural language sentences.  Next, we can fine-tune our models on the data from NDH.  NDH was introduced as a task by The Cooperative Vision and Dialogue Navigation Dataset (CVDN) where dialogue histories are collapsed to form a long input instruction similar to the VLN formulation.  

%CVDN is comprised of 2050 dialogues between two human speaker-follower players where the goal is for the follower to reach the closest location with the target object as quickly as possible. Each dialogue is a sequence of question-answer interactions covering nearly 7,000 different trajectories in 83 Matterport indoor environments. The goal of the conversation is to find a target location which is specified up front in natural language (e.g. a fire-extinguisher).  In CVDN, all targets are both ambiguous and underspecified to force dialogue and overcome basic structural priors (e.g. toilets are in bathrooms). In practice, this means that no step-by-step instructions are provided or immediately deducible from the start without asking for help. NDH refers to the task of treating the dialogue history as a static set of instructions (a la VLN) and several recent papers have focused on performing this task \cite{xin,cvdn}.

%Our aims are more ambitious, we not only want an agent to understand a static dialogue but to generate its own.  To do this, we will train our models $\mathcal{N}, \mathcal{Q}$, and $\mathcal{O}$ on their respective roles in the data, but all gold information will be discarded during evaluation.  To ensure we maintain a fair comparison for upper-bound human performance, we will evaluate with the same house scans \textit{S}, starting position starting position $p_0$, and the target object $t_o$.  In this way we can directly compare the quality of our dialogues quantitatively (e.g. how far are we from goal and how many questions did we require?).  We analyze this in detail in Section \ref{sec:analysis}.
%CVDN identifies as targets a set of 81 different objects that are common and appear 2 or more times in at least 5 different Matterport indoor environments. The initial dialogue prompts include the house scan \textit{S}, the starting position $p_0$, and the target object $t_o$. 


%\subsection{Evaluation Metrics}
%For evaluation of the agent, we use the goal progress which refers to the amount of distance in meters covered from the starting position to the goal location along the shortest path. As for the speaker, we use the BLEU score between the generated dialogue history and the ground truth human dialogue for the trajectory. It should be noted that due to noise in the data like wrong human instructions, it is not necessarily always desirable to get a BLEU score of 1.0 at the expense of lower agent performance.



## 4 

%\subsection{Implementation details}
%As previously done in vision language navigation\cite{vln}, we use as image features $\Tilde{f}$ the output from the last convolutional layer of ResNet\cite{resnet} trained on ImageNet\cite{imagenet}. 
%These image features are not changed during training or testing.

%\subsubsection{Pre-training NDH task on CVDN.} 
%Leveraging results from meta-learning\cite{maml} where meta-learning leads to faster adaptation of deep networks, we pre-train the NDH task on the CVDN dataset.
%For pre-training, the agent is allowed to see the entire dialogue history from the start. However, no new questions or answers are generated while the agent is training. 
%Figure ~\ref{fig:action_decoder} illustrates how action decoding is done at each time step. Before the agent is placed in the environment,
%the entire dialogue history is feed in to an LSTM encoder with a word embedding size of 256,
%a hidden size of 512, training dropout ratio of 50\%, and max input length of 160 tokens. 
%The LSTM encoder outputs a hidden state $\Tilde{h}_{t-1}$ and a context $[u_1,...,u_j]$ where each $u_j$ corresponds to an encoded
%instruction token. The context $[u_1,...,u_j]$ is constant because in the NDH task, the instructions do not change. Then at each time step, the decoder takes in the previous action $\Tilde{a}_{t-1}$,
%which initially is \textit{start}, the current panorama features $\Tilde{f}_t$, and the k navigable viewpoint features $\Tilde{g}_{t,k}$. The decoder is an attentive LSTM Decoder as shown in figure \ref{fig:action_decoder}. Action embedding size and target embedding size are 32. 



% \subsection{The Navigation from Dialogue History Task (NDH)}

% as shown in equation \ref{eq:cross_entropy}.  

% \begin{align}
%   CE(X,Y) & = -\sum_{i}^{C} y_i \ log \ (\textbf{Softmax}(x)_i) \label{eq:cross_entropy}
% \end{align}
%\subsection{The Collaborative Vision Dialogue Navigation Task}
%Traditionally, in Vision-Language Navigation, the agent has full access to instructions from start to finish. 
%However, having access to these instructions is not sufficient. 
%Agents that get lost along the way may suffer from having misaligned instructions.
%Instead, a more realistic scenario for Collaborative Vision Dialogue Navigation is to allow the agent 
%to ask for help in the form of a question and get a response in the form of an answer as the agent
%acts upon its environment. This new approach is the Collaborative Vision Dialogue Navigation gameplay 
%illustrated below. \\
%
%%\begin{wrapfigure}[5]{l}{\linewidth}
%%\centering
%%\vspace{-25pt}
%%\caption{Illustration of gameplay}
%%\vspace{-5pt}
%%\includegraphics[width=\linewidth]{images/gameplay.JPG}
%%\label{fig:gameplay}
%%\end{wrapfigure}
%
%Under this formulation, the agent starts only with egocentric 
%knowledge of the objects in front of it and the target it needs to reach. 
%Its only actions are to move forward, turn up, down, left, or right. 
%At any point in time, the agent may recognize it got lost and ask a question.
%The question is generated by paying attention to the images at the viewpoint where the agent decided to ask the question.
%In order to reply to that question, the speaker looks a the next five steps in the shortest path to the goal
% then, by attending to the images along this path, samples word-by-word to generate a text answer.
% With the new question-answer pair, the agent updates its context to predict the next action.
% The agent may choose to save its dialogue history in which case the entire previous dialogue history along
% with the new question and answer are used to update the context.
% Finally, the rollout ends when the agent decides to stop. 

%We generate additional data by sampling from a navigator model and allowing it to get lost.
%To augment the data, during training, each regular agent rollout also generates trial runs with different actions sampled based on the sampling or action-choosing technique being used. Also full dialog histories are generated out of these trial runs. One of the trial runs is the one where instead of sampling, the agent selects the argmax action from its predicted logits. This ensures that the best trial run will perform no worse than the argmax. Once these trial runs are generated, the one with the greatest goal progress is selected to do training on where the generated data is treated as ground truth and trained on.

%As another way to augment the data, we leverage the technique of random start where the agent can start anywhere in the simulator as long as the starting viewpoint has at least one viable path to the goal. In order to guarantee that the new starting position can reach the goal we introduce a \textit{Jitter} parameter that determines how far is the new starting position expected to be from the original initial position. For instance, a \textit{Jitter} of 1 indicates that the new starting position is a neighbor of the original starting position.


When the agent asks a question, words are sampled word-by-word but instead of only generating a single question, we generate $N$ candidate questions.
Then, when generating answers for each candidate question, we generate $N$ candidate answers. This produces a total of $N^2$ 
different candidate question-answer pairs. In order to choose which of these pairs is expected to get the agent closest to the end goal, 
an \acronymnormal\ is run for each pair. Inside the \acronymnormal\ a previous version of the agent is run to completion.
As it runs, this \acronymnormal\ agent may potentially ask a question which would trigger a recursive call to a new \acronymnormal .\
This recursive process continues until the \acronymnormal\ agent decides to stop. To prevent a potentially infinite number of \acronymnormal s,
the branching factor may change to prevent going above a certain computational limit. 
At any given point in time, there are at most $N^2$ different candidate question-answer pairs being mentally run. 
This is achieved by decreasing the branching factor from $N$ to 1 on subsequent recursive calls. 
Once all the $N^2$ candidates decide to stop, the model picks the answer for which the \acronymnormal\ agent got closest to the goal.
This answer is then returned to the original agent as the best answer. The original agent updates its saved dialogue history and continues it rollout.
A new question may be asked which would once again trigger the creation of \acronymnormal s.\ 
This continues until the original agent decides to finally stop. \\
By exposing the goal progress metric to the speaker, the \acronymnormal\ also allows the speaker to leverage Reinforcement Learning techniques.
This is an novel approach with much to be explored. 
In particular, this paper shows the effects of training the speaker with the cross entropy loss between the human and the generated dialogues added to the best-answer \acronymnormal\ RL agent loss.


\subsection{Experiments}

\subsubsection{CVDN Gameplay Baseline} In the CVDN task, the only initial input is the target, 
so after pre-training with the NDH task, we follow the same action decoding scheme as in figure \ref{fig:action_decoder}.
However, the context $[u_1,...,u_j]$ is no longer fixed. The dialogue history starts as only the target but increases 
as more questions are asked and answered. The hidden state $\Tilde{h}_{t-1}$ is not cleared out on each context change.
We use a batch size of 10 and train for 20000 iterations.
Also, since the average number of steps between questions is 4.46, we use 4 as the number of steps between each
question and leave the exploration on when to ask a question and topic of future work.
Furthermore, since questions are generated and answered as the agent is interacting with the environment it is also possible to train the 
speaker as it generates new responses. The baseline of CVDN gameplay; however, does not train the speaker beyond the pre-training.
The Data Augmentation and \acronymnormal\ models do train the question and answer generation system. \\
Figure \ref{fig:instruction_decoder} illustrates how instruction decoding is done. It should be noted that the model that generates questions is the same as the model that generates answers, the only difference between the two is that when generating questions, we start the sequence with the \textit{$<$NAV$>$} tag and use only the current viewpoint as input features whereas to generate an answer we start the sequence with the  \textit{$<$ORA$>$} tag and use the visual features from the next 5 viewpoints along the shortest path to the goal.

% \begin{figure}
%\centering
%\includegraphics[width=\linewidth]{images/instruction_decoder.JPG}
%\caption{Illustration of Seq2Seq instruction decoding}
%\label{fig:instruction_decoder}
%\end{figure}

%\subsubsection{Data Augmentation} 
%In the data augmentation model, on each iteration we do teacher forcing as in the original CVDN Baseline formulation but with speaker training and filter from 3 trials runs for the one that had a final distance closest to the goal. On each trial run, we output to a log file the trajectory and generated dialogue history. One of the trial runs uses the argmax from the predicted action logits while the rest sample for the next action. In practice, each trial run has a standard deviation of about 3 meters. From the log file we filter for the run that got closest to the goal and train on the output from this best run adding $\lambda$\% of this augmented loss to the total loss. The analysis section has an exploration of this $\lambda$ parameter but, in short, we found $\lambda=0.1$ to work best. We find that without including the argmax as a trial run and with no $\lambda$ parameter, the speaker quickly starts to deviate away from English language leading to worse performance. 
%\subsubsection{\acronymnormal} 
%As the name implies, \acronymnormal\ is implemented recursively. 
%On every four time steps, the agent generates 3 sampled word-by-word questions each of which leads to 3 sampled candidate answers for a total of 9 question-answer pairs. For each question-answer pair, the speaker loads a previous instance of the agent as a Mental Model with the  question-answer pair concatenated to its dialogue history. As it rolls out, after every 4 steps, the Mental Model agent may also ask for a question at which point another mental model agent is run with a newly sampled question-answer pair concatenated to its dialogue history but with a single candidate instead of 9. This interaction of going deeper and deeper into the recursive stack continues until the last-layer Mental Model agent decides to stop or reaches the maximum limit of 80 episodes. Once at the last layer, the top-most mental model agent returns its goal progress which propagates recursively all the way back to the first recursive call. With the goal progresses from the 9 Mental Models, the speaker can pick the answer and question which led to the most goal progress. The original agent, then receives the new question-answer pair, concatenates it to its dialogue history and continues its rollout once again asking for help at the next 4 time steps which will lead to 9 new Mental Models and so on until the original agent decides to stop or runs out of episodes.
%
%\subsection{Action Probabilities}
%In order to select the best question-answer pair from the candidates on each mental model run, during evaluation instead of using the Goal Progress, the agent leverages the average of its last action probabilities as a signal. This way, the model picks the question-answer pair for which the respective mental model was most confident out of all the candidates.


## 5

% \subsection{Analysis on Data Augmentation}
% \subsubsection{Contribution of Data Augmentation}
% Fig.~\ref{fig:gp_vs_iter} for Goal Progress vs iteration for different lambdas of data augmentation
% % \subsubsection{Temperature Sampling}
% % Fig.~\ref{fig:temperature} illustrates Goal Progress vs number of Data augmentation teacher forcing rounds
% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{images/gp_vs_iter.JPG}
% \caption{Data Augmentation Goal Progress vs  Iteration}
% \label{fig:gp_vs_iter}
% \end{figure}
% 
% % \begin{figure}
% % \centering
% % \includegraphics[width=\linewidth]{images/gp_vs_aug.JPG}
% % \caption{Goal Progress vs Data Augmentation Rounds}
% % \label{fig:temperature}
% % \end{figure}
% \subsubsection{Random Start}
% \subsection{Analysis on \acronymnormal}




%\setlength{\tabcolsep}{4pt}
%\begin{table}
%\centering
%\caption{Gameplay results on NDH}
%\label{table:results}
%\begin{small}
%\begin{tabular}{lclclclclclc}
%\hline\noalign{\smallskip}
%\textbf{Fold} & \textbf{Model} & \textbf{Input} & \multicolumn{2}{c}{\textbf{Generated}} & \textbf{Goal Progress(m)} & \textbf{BLEU} \\
%  &   & $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$&$\uparrow$&$\uparrow$\\
%\hline \noalign{\smallskip}
%\multirow{16}{*}{\rotatebox[origin=c]{90}{Val Seen}}  &  \multirow{4}{*}{Baseline} &\multicolumn{3}{c}{Shortest Path Agent}& 9.359 & 1.0\\
%& & \ding{51} & & & 1.733 & None\\
%& & \ding{51} & \ding{51} & & 1.688 & 0.0383\\
%& & \ding{51} & \ding{51} & \ding{51} & 1.662 & 0.0386 \\
%\cline{2-7}& \multirow{3}{*}{Data Aug} & \ding{51} & & & 2.632 & None\\
%& & \ding{51} & \ding{51} & & 2.519 & 0.0298\\
%& & \ding{51} & \ding{51} & \ding{51} & 1.358 & 0.0328\\
%\cline{2-7} \noalign{\smallskip} & Data Aug & \ding{51} &  & & - & None\\
%& + & \ding{51} & \ding{51} & & - & -\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \multirow{3}{*}{\acronymnormal} & \ding{51} &  &  & - & None\\
%& & \ding{51} & \ding{51} & & - & -\\
%& & \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \acronymnormal & \ding{51} &  &  & - & None \\
%& + & \ding{51} & \ding{51} & & - & -\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\hline
%\noalign{\smallskip}
%\multirow{16}{*}{\rotatebox[origin=c]{90}{Val Unseen}}  &  \multirow{4}{*}{Baseline} &\multicolumn{3}{c}{Shortest Path Agent}& 9.831 & 1.0\\
%& & \ding{51} & & & 0.184 & None\\
%& & \ding{51} & \ding{51} & & 0.216 & 0.0382\\
%& & \ding{51} & \ding{51} & \ding{51} & 0.398 & 0.0365\\
%\cline{2-7}& \multirow{3}{*}{Data Aug} & \ding{51} & & & 0.387 & None\\
%& & \ding{51} & \ding{51} & & 0.350 & 0.0419\\
%& & \ding{51} & \ding{51} & \ding{51} & \textbf{0.484} & \textbf{0.0423}\\
%\cline{2-7}\noalign{\smallskip} & Data Aug & \ding{51} &  &  & - & None\\
%& + & \ding{51} & \ding{51} & & - & -\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \multirow{3}{*}{\acronymnormal} & \ding{51} &  &  & - & None\\
%& & \ding{51} & \ding{51} & & - & -\\
%& & \ding{51} & \ding{51} & \ding{51} & - & -\\
%\cline{2-7}\noalign{\smallskip}& \acronymnormal & \ding{51} &  &  & - & -\\
%& + & \ding{51} & \ding{51} & & - & None\\
%& Random Start& \ding{51} & \ding{51} & \ding{51} & - & -\\
%\hline
%\end{tabular}
%\end{small}
%\end{table}


## Appendix

% \setlength{\tabcolsep}{4pt}
% \begin{table}
% \centering
% \caption{Generated Conversations}
% \label{table:conversations}
% \begin{small}
% \begin{tabular}{lcp{10.6cm}}
% \toprule
%  & & Conversation \\
% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{Human}} & Q:& Should I head into the room with the table ?\\
% & A:& head into the room with the table, turn to the left and head down the hall to the stairs \\ 
% \midrule
% \multirow{11}{*}{\rotatebox[origin=c]{90}{Baseline}} & Q:& i am lost . where should i go next ? \\
% & A:& turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go into the bedroom . go through the door to your right . go through the door to your right , move forward forward on your right .\\
% & Q:& i am lost . where should i go next ? \\
% & A:& exit the room . turn right and go through the door on the right .  go through the first door on your right .\\
% & Q:& i am lost . where should i go next ?\\
% & A:& go to the right . go to the stairs . go up the stairs . yes , go forward forward on the right .\\
% \midrule
% \multirow{9}{*}{\rotatebox[origin=c]{90}{Data Augmentation}} & Q:& i am lost . where should i go next ?\\
% & A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
% & Q:& i am lost . where should i go next ?\\
% & A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
% & Q:& i am lost . where should i go next ?\\
% & A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
% \midrule
% \multirow{11}{*}{\rotatebox[origin=c]{90}{\acronymnormal}} & Q:& this is not the room . should i go through the door , the open doorway , or up the stairs ?\\
% & A:& go out the open door in front of you . you should see a dining table to your right as you exit \\
% & Q:& should i go toward the green door , the open doorway , or up the stairs ? \\
% & A:& you will see a few stairs to your right as you exit \\
% & Q:& where should i go from here ? \\
% & A:& left past the plant . \\
% & Q:& i am in the bathroom at the bottom of the stairs .  should i move or toward the bedroom ? \\
% & A:& left and then right in the room that will be on the desk \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{table}
% \setlength{\tabcolsep}{1.4pt}

\subsubsection{Pre-training on R2R and NDH}

Table~\ref{table:pretrain} shows results from pre-training of agent and speaker
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Pre-training results on NDH}
\label{table:pretrain}
\begin{tabular}{lcccccc}
\hline\noalign{\smallskip}
\textbf{Fold} & \textbf{Task(s) Trained} & \multicolumn{3}{c}{\textbf{Seq-2-Seq Input}} & \textbf{Goal Progress} & \textbf{BLEU} \\
  &   & $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$&$\uparrow$&$\uparrow$\\
\hline \noalign{\smallskip}
\multirow{4}{*}{\rotatebox[origin=c]{90}{Val Seen}} &   &\multicolumn{3}{c}{Shortest Path Agent}& 9.359 & 1.0\\
 & NDH  & \ding{51} & \ding{51} & \ding{51} & 5.92  & None\\
 \cline{2-7} \noalign{\smallskip} & NDH follower  & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{5.261} & \multirow{2}{*}{\textbf{0.0009}}\\
  & R2R + NDH speaker & & & &\\
\hline
\noalign{\smallskip}
\multirow{2}{*}{\rotatebox[origin=c]{90}{Val Unseen}}  &   &\multicolumn{3}{c}{Shortest Path Agent}& 9.831 & 1.0\\
& NDH   & \ding{51} & \ding{51} & \ding{51} & 2.10  & None \\
\cline{2-7} \noalign{\smallskip} & NDH follower  & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{2.018} & \multirow{2}{*}{\textbf{0.0007}}\\
  & R2R + NDH speaker & & & &\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.9pt}




Table~\ref{table:cvdn_rl} shows follower RL vs full RL results on CVDN
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Follower RL vs full RL results on CVDN}
\label{table:cvdn_rl}
\begin{tabular}{cccccccc}
\hline\noalign{\smallskip}
\multicolumn{2}{c}{\textbf{Fold}} &  \multicolumn{2}{c}{\textbf{Generated}} &
\multicolumn{2}{c}{\textbf{RL Trained}} & \textbf{Goal Progress} & \textbf{BLEU} \\
  & & $Q_i;A_i$& $Q_{i-1};A_{i-1}$& A2C& Speaker &$\uparrow$&$\uparrow$\\
\hline \noalign{\smallskip}
\multirow{2}{*}{Val Seen} &  & \ding{51} & \ding{51} & \ding{51} & & - & - \\
  &   & \ding{51} & \ding{51} & \ding{51} & \ding{51} & - & -\\

\hline
\noalign{\smallskip}
\multirow{2}{*}{Val Unseen}  &  & \ding{51} & \ding{51} & \ding{51} &  & - & -\\ 
  &   & \ding{51} & \ding{51} & \ding{51} & \ding{51} & - & - \\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.9pt}

\setlength{\tabcolsep}{4pt}
\begin{table}
\centering
\caption{Gameplay results on NDH}
\label{table:results}
\begin{small}
\begin{tabular}{llcccccc}
\toprule
 & \textbf{Model} & \multicolumn{3}{c}{\textbf{Goal Progress (m) $\uparrow$}} & \multicolumn{3}{c}{\textbf{\textbf{BLEU} $\uparrow$}} \\
  &   & $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$& $t_0$& $Q_i;A_i$& $Q_{i-1};A_{i-1}$\\
\hline \noalign{\smallskip}
\multirow{6}{*}{\rotatebox[origin=c]{90}{Val Seen}}  &  
  Shortest Path &       &       & 9.359 &      &        & --\\
& Baseline      & - & - & - & -- & - & -\\
& DA      & - & - & - & -- & - & - \\
& DA + RS &       &       &       & -- &        & \\
\cline{2-8}   
& \acronymnormal        &       &       &       & -- &     &\\
& \acronymnormal{} + RS &       &       &       & -- &     & \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{Val Unseen}}  &  
  Shortest Path &       &       & 9.831 &      &        & --\\
& Baseline      & - & - & - & -- & - & -\\
& DA            & - & - & - & -- & - & - \\
& DA + RS       &       &       &       & --   &        & \\
\cline{2-8}   
& \acronymnormal        &       &       &       & -- &     &\\
& \acronymnormal{} + RS &       &       &       & -- &     & \\
\bottomrule
\end{tabular}
\end{small}
\end{table}
\setlength{\tabcolsep}{1.9pt}



\begin{align}
  CE(X,Y) & = -\sum_{i}^{C} y_i \ log \ (\textbf{Softmax}(x)_i) \label{eq:c_e}\\
  & where \quad \textbf{Softmax}(x)_i = \frac{e^{x_i}}{\sum_{j}^{C}e^{x_j}}
\end{align}


\setlength{\tabcolsep}{4pt}
\begin{table}
\centering
\caption{Generated Conversations}
\label{table:prev_conversations}
\begin{small}
\begin{tabular}{lcp{10.6cm}}
\toprule
 & & Conversation \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Human}} & Q:& Should I head into the room with the table ?\\
& A:& head into the room with the table, turn to the left and head down the hall to the stairs \\ 
\midrule
\multirow{11}{*}{\rotatebox[origin=c]{90}{Baseline}} & Q:& i am lost . where should i go next ? \\
& A:& turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go straight down the hallway . turn right and go into the bedroom . go through the door to your right . go through the door to your right , move forward forward on your right .\\
& Q:& i am lost . where should i go next ? \\
& A:& exit the room . turn right and go through the door on the right .  go through the first door on your right .\\
& Q:& i am lost . where should i go next ?\\
& A:& go to the right . go to the stairs . go up the stairs . yes , go forward forward on the right .\\
\midrule
\multirow{9}{*}{\rotatebox[origin=c]{90}{Data Augmentation}} & Q:& i am lost . where should i go next ?\\
& A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
& Q:& i am lost . where should i go next ?\\
& A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
& Q:& i am lost . where should i go next ?\\
& A:& walk down the stairs . turn left and walk down the stairs . stop at the top of the stairs .\\
\midrule
\multirow{11}{*}{\rotatebox[origin=c]{90}{\acronymnormal}} & Q:& this is not the room . should i go through the door , the open doorway , or up the stairs ?\\
& A:& go out the open door in front of you . you should see a dining table to your right as you exit \\
& Q:& should i go toward the green door , the open doorway , or up the stairs ? \\
& A:& you will see a few stairs to your right as you exit \\
& Q:& where should i go from here ? \\
& A:& left past the plant . \\
& Q:& i am in the bathroom at the bottom of the stairs .  should i move or toward the bedroom ? \\
& A:& left and then right in the room that will be on the desk \\
\bottomrule
\end{tabular}
\end{small}
\end{table}
\setlength{\tabcolsep}{1.4pt}



### Old 


%% %\setlength{\tabcolsep}{4pt}
%% \begin{table*}
%% \centering
%% \begin{small}
%% \begin{tabular}{ll@{\hspace{2em}}cc@{\hspace{2.5em}}ac@{\hspace{2.5em}}ca}
%%  & \textbf{Model} & \multicolumn{4}{c}{\textbf{Goal Progress (m) $\uparrow$}} & \multicolumn{2}{c}{\textbf{\textbf{BLEU} $\uparrow$}} \\
%% \toprule
%%   &   & $t_0$& $QA_i$& $QA_{i-1:0}$& \begin{scriptsize}\begin{tabular}{@{}c@{}}+\! Oracle\\Stopping\end{tabular}\end{scriptsize} & $QA_i$& $QA_{i-1:0}$\\
%%   \midrule
%% \multirow{5}{*}{\rotatebox[origin=c]{90}{Val Seen}}  
%% & Baseline                       &\textbf{20.11}& 10.52      & \Be{14.96}     & \textbf{22.9} & 0.9    & 0.8     \\
%% & Data Augmentation                      & 20.11    & 10.51      & 10.04     & 14.2 & 1.3    & 1.3     \\
%% %& DA + RS                       &\Be{20.48}& 10.80      & \Be{15.01}&      & 1.3    & 0.3     \\
%% & \acronym$_{N=1}$               &18.73     & 10.02      & 13.27     & 20.4 & 3.3    & 3.0     \\
%% %& \acronym$_{N=1}$ +RS          &19.82     & 10.57      & 11.51     & --   &\Be{3.5}& 3.1     \\
%% & \acronym$_{N=3}$ +AP           &18.90     & \textbf{11.54} & 13.97 & 16.8 &\textbf{3.4}&\Be{3.6}\\
%% %\cline{2-8}   
%% %& Perfect \acronym$_{N=3}$      &18.90     & 7.42       & 11.00     & -- & 3.4    & 3.5 \\
%% %& Perfect \acronym$_{N=3}$ + RS &15.64     & 9.48       & 11.61     & -- & 3.5    & 3.3\\
%% &  Shortest Path                 & \multicolumn{4}{@{}c}{----------- 32.79 ----------- }    &   & \cellcolor{white}\\
%% \midrule
%% \midrule
%% \multirow{5}{*}{\rotatebox[origin=c]{90}{Val Unseen}}    
%% & Baseline                           & 6.78     & 4.67      & \PZ4.55      & 6.34& 0.5  & 0.5\\
%% & Data Augmentation                                 & 6.78     & 5.47      & \PZ4.38      & 6.52& 1.3  & 1.1\\
%% %& DA + RS                           & 4.408    & \Be{6.15} & \PZ3.07      & --  & 1.2  & 0.3\\
%% & \acronym$_{N=1}$                   & 6.10     &\textbf{6.09}  & \PZ5.11      & 5.95 & 2.6  & 2.8\\
%% %& \acronym$_{N=1}$ +RS              & 5.838    & 5.488     & \PZ6.24      & --  & 2.9  & 2.7\\
%% & \acronym$_{N=3}$ +AP               &\textbf{7.26} & 5.53      & \PZ\Be{5.61} &\textbf{8.87} &\textbf{2.9}&\Be{2.9}\\
%% %\cline{2-8}          
%% %& Data Aug. \hspace{8pt} + O Stop   &          &           & \PZ6.52      &     &      &      \\
%% %& \acronym$_{N=3}$ +AP + O Stop     &          &           & \PZ8.87      &     &      &      \\
%% %& \acronym$_{N=3}$ + O branch       &          &           & \PZ8.16      & --  & 2.9  & 2.9\\
%% %& \acronym$_{N=3}$ + O branch       &   7.26   & 8.11      & \PZ8.16      & --  & 2.9  & 2.9\\
%% %& Perfect \acronym$_{N=3}$ + RS     &   6.098  & 7.563     & \PZ7.01      & --  & 2.8  & 2.9\\
%% & Shortest Path                     & \multicolumn{4}{@{}c}{----------- 29.32 ------------}                & & \cellcolor{white} \\
%% \bottomrule
%% \end{tabular}
%% \end{small}
%% \caption{Gameplay results on CVDN -- All results evaluated when agent voluntarily stops or at 80 steps.}
%% \label{table:cvdn_results}
%% \end{table*}



%\paragraph{Initial Models}
%In Table \ref{table:pretrain_cvdn} we see that this initialization works well on seen navigation environments.  In contrast, while pretraining does help our final speaker models, note that the generation task for NDH is substantially more difficult than seen in the literature for VLN.  This is likely due to longer sequences and co-reference.

% \begin{table}
% \begin{small}
% \begin{center}
% \begin{tabular}{lccccc}
% \hline\noalign{\smallskip}
% \textbf{Fold} & & \textbf{Goal Progress}$\uparrow$ & \textbf{BLEU}$\uparrow$ \\
% \hline \noalign{\smallskip}
% \multirow{2}{*}{Seen}  & Gold  & 32.789 & -- \\
%                        & Pretraining & 20.840  & 0.20\\
% \midrule
% \noalign{\smallskip}
% \multirow{2}{*}{Unseen}  & Gold & 29.321 & -- \\
%                          & Pretraining & 6.550  & 0.19 \\
% 
% \hline
% \end{tabular}
% \end{center}
% \end{small}
% \caption{Performance of initial models on navigating from and generating full dialogues during pretraining.}
% \label{table:pretrain_cvdn}
% \end{table}



%\paragraph{Stopping Criteria}
%Under this implementation, the agent can only stop when it either voluntarily decides to predict the STOP action or when it runs out of steps. Previous work \cite{cvdn}  has used a max length of 80 steps; therefore, in this paper we also have this limit. It should be noted that because of this restriction results may not be as optimal as in the case when the agent has a known per-trajectory maximum number of steps.   


%# Seen      CSV     Homero
%baseline = [19.85, 10.06]
%dataaugm = [10.09, 10.00]
%rmmn1    = [15.53, 11.00]
%rmmn3    = [13.81, 14.13]
%print(ave(baseline), ave(dataaugm), ave(rmmn1), ave(rmmn3))
% 14.96 10.04 13.27 13.97
%
%# Unseen    CSV   Homero
%baseline = [3.44, 5.67]
%dataaugm = [4.19, 4.58]
%rmmn1    = [3.94, 6.28]
%rmmn3    = [5.34, 5.88]
%print(ave(baseline), ave(dataaugm), ave(rmmn1), ave(rmmn3))
%  4.55  4.38  5.11  5.61


